Personalized Emphasis Framing for Persuasive Message Generation

In this paper, we present a study on personalized emphasis framing which can be used to tailor the content of a message to enhance its appeal to different individuals. With this framework, we directly model content selection decisions based on a set of psychologically-motivated domain-independent personal traits including personality (e.g., extraversion and conscientiousness) and basic human values (e.g., self-transcendence and hedonism). We also demonstrate how the analysis results can be used in automated personalized content selection for persuasive message generation.

==> EMNLP2016 - arxiv/Conclusion.tex <==
 \section{Discussion: Domain Generalization}
In general, there are two main challenges in adapting a personalized content selection model trained in one domain to another domain: (1) adapting the {\it data model} from one domain (e.g., restaurant data) to another (e.g., movie data);  (2) adapting a domain-specific {\it user model} (e.g., a user' preferences of restaurant features such as "cuisine type") to a different domain (e.g., a user's preferences of movie features such as "movie genre").  Although our current model is trained in the automobile domain, we adopted a domain-independent user model motivated by psychological theories(e.g., personality and basic human values), instead of using domain-dependent user preference models (e.g, a user's preferences of "fuel economy"). This has made our work much more generalizable than systems that rely on domain-dependent user properties. Moreover, to make our current findings more generalizable, we can apply typical domain adaptation methods such as instance-based~\cite{zadrozny04}  or feature-based transfer learning~\cite{Blitzer06} to further adapt the current results.
  
 \section{Conclusions}
In this study, we analyzed the relationship between an individual's traits and his/her perceived aspect importance. Our analysis has uncovered interesting patterns that can be used to automatically customize a message's content to enhance its appeal to an individual.  We also proposed a cascade content selection model to automatically incorporate the analysis results in automated persuasive message generation. Our evaluation results have demonstrated the effectiveness of this approach. 

==> EMNLP2016 - arxiv/Experiment.tex <==
\section{Learning  Emphasis Framing Strategies}

The goal of this study is to derive emphasis framing patterns based on a receiver's traits and his/her aspect selection decisions.  
\subsection{Data Collection}
We designed another HIT (Task 3) on AMT to collect the data needed for the study. In Task 3, each Turker was asked to take the IPIP and PVQ surveys so that we can obtain their Big5 personality and value scores. In addition, we also asked them to rank all eight car aspects based on their importance to them.  To control the influence of the value of a car aspect on a user's aspect selection decision (e.g.,  if the value of ``safety" is ``poor"  and the value of ``fuel economy" is ``good",  to promote the car, people almost always describe it as "a car with good fuel economy", not  ``an unsafe car", regardless of a receiver's personality). In this study, we kept the values of all car aspects unspecified. After removing the invalid data,  our dataset has 594 valid responses, each contains a Turker's personality and value scores as well as his rank of the eight car aspects.
%or the same. Specifically, we asked  the Turkers to perform three subtasks: (1) Rank all the car aspects with unspecified values (e.g., whether they consider "safety" more important than  "fuel economy").   (2) Rank all the car aspects when their values are all "5" (3) Rank all the car aspects when their values are all "1". To make the tasks more intuitive for the Turkers, in subtask 2,  we presented each Turker eight car descriptions, each focused on only one aspect and we asked the Turkers to rank these cars based on their preferences (e.g, please rank the following cars based on your preferences (a) a very safe car (b) a very cheap car etc.). For subtask 3, we also presented the Turkers eight car descriptions, each focused on only one car aspect, we asked them to rank the cars based on their concerns (e.g., please rank the following cars based on how much you want to avoid them (a) a very unsafe car (b) a very expensive car etc.). With these three subtasks, we want to assess  (1) whether personal traits play a role in a Turker's decision of important car aspects (2) the impact of aspect value on their decisions (high values in subtask 2 and low values in subtask 3.  
%To determine whether the questions in the three subtasks measures different constructs or they all measures the same underlying construct, and thus can be loaded into a single latent factor, we  computed Cronbach's alpha to  determine their internal consistency.  Table~\ref{tbl:featureMsgconsistency} shows the computed Cronbach's alpha ~\cite{Cronback1951} for each of the eight car aspects. A value of 0.7 or higher is considered acceptable as a good indication of reliability ( Nunnally \& Bernstein, 1994). Since all the $\alpha$s  are 0.7 or higher, in the following, we focus on feature ranks with unspecified value since it has the strongest association to the underlying latent factor.
In the following, we describe how we analyze the relationship between aspect rank and personal traits. 
%J.C. Nunnally, I.H. Bernstein Psychometric theory (3rd ed)McGraw-Hill, New York (1994)
%Cronbach, L. J. (1951). Coefficient alpha and the internal structure of tests. Psychometrika. 16, 297-334.
%\subsection{Data Preparation}
%To validate the reliability of our data, we computed Spearman's rank correlation $r$ coefficients between feature and message selection. We found rank orders of features and message with good feature are highly correlated with $r=0.81$. The rank orders of features and message with good feature are moderately correlated with $r=0.64$. The reliability is acceptable.
%\begin{table}[h]
%\label{tbl:featureMsgCorrealtion}
%\centering
%\caption{Correlation Measurement}
%\begin{tabular}{|c|c|} \hline
%  &Correlation\\ \hline
%Feature vs Message 1 & 0.81\\ \hline
%Feature vs Message 2 & 0.64\\ \hline
%Message 1 vs Message 2 & 0.67\\ \hline
%\end{tabular}
%\end{table}
%We also measured the internal consistency within three groups. Internal consistency describes the extent to which all the items in a test measure the same concept or construct and hence it is connected to the inter-relatedness of the items within the test\cite{tavakol2011making}. We used Cronbach's $\alpha$ to measure how closely related a set of items are as a group. For all features, $\alpha$ is higher than 0.7 which is considered as acceptable internal consistency within these three groups. We do not have to consider three groups separately in our following experiments, we thus only focus on feature preference.
%\begin{table}[h]
%\small
%\label{tbl:featureMsgconsistency}
%\caption{ Consistency Analysis }
%\centering
%\begin{tabular}{|c|c|} \hline
%Feature & $Cronback's \alpha$ \\ \hline
%Safety & 0.81	\\ \hline
%Fuel & 0.84	\\ \hline
%Quality & 0.79	\\ \hline
%Style & 0.79	\\ \hline
%Price & 0.78	\\ \hline
%Luxury & 0.78	\\ \hline
%Performance & 0.82\\ \hline	
%Durability & 0.81\\ \hline
%\end{tabular}
%\end{table}
%To categorize the people based on traits, we converted the original score of traits to percentile score which indicate the percentage of the people who score less than you on the dimension in our reference population. For example, if percentile score of \emph{Extroversion} is 15, which means that about 15 percent of the people in our comparison sample are less extraverted than you, in other words, you are rather introverted. We defined 20\% as threshold, if percentile score of \emph{Extroversion} is below 20\%, you are considered as introvert; if percentile score of \emph{Extroversion} is above 80\%, you are considered as extrovert. Table \ref{tbl:readerdist} shows the how users are polarized in our data according to different traits.
%\input{tbl/tbl_readerdist}
\subsection{Pattern Discovery with Regression}
\input{tbl/tbl_regression}
In our first study, we employed regression analysis to identify significant correlations between personal traits and aspect ranks. Specifically, we trained eight linear regression models, one for each of the eight car aspects. The dependent variable in each model is the rank of an aspect (from 1 to 8) and the independent variables are the ten user traits.  Here we only focused on the main effects since a full interaction model of ten traits will require more data to train.  Since the raw scores of  the personality and the value traits use different scales, we normalized these scores so that they are all from 0 to 1. Table ~\ref{tbl:regression} shows the regression results. 
Several interesting patterns were discovered in this analysis:  (a)  a positive correlation between the rank of  ``luxury" and ``self-enhancement", a trait often  associated with people who pursue self-interests and value social status, prestige and personal success ($p<0.0001$). This pattern suggests that to promote a car to someone who scores high on ``self-enhancement", we need to highlight the ``luxury" aspect of a car.  (b) the importance rank of ``safety" is positively correlated with ``conservation", a trait associated with people who conform to tradition and pursue safety, harmony, and stability ($p<0.005$). This result suggests that for someone values ``conservation", it is better to emphasize ``car safety" in a personalized sales message. (c)  ``self-transcendence", a trait often associated with people who pursue the protection of the welfare of others and the nature, is positively correlated with the rank of ``fuel economy" ($p<0.005$) but negatively correlated with the rank of ``style" ($p<0.005$). This suggests that for someone who values ``self-transcendence", it is better to emphasize ``fuel economy", but not so much on ``style".  Other significant correlations uncovered in this analysis include a negative correlation between car ``price" and ``conservation" ($p<0.005$), a negative correlation between car ``safety" and ``conscientiousness" ($p<0.05$), and a positive correlation between ``openness to change" and car ``performance" ($p<0.05$). 
%The formula is given as: \\
%\begin{align}
%x^{'}= \frac{x - min(x)}{max(x) - min(x)}
%\end{align} 
%So far,  we have only considered the main effects in the regression analysis. In the following, we further explore methods that allow us to uncover interesting high-order interaction patterns between different traits. 
%In these models, we take main effects into consideration without interactions. We only find one significant correlation in 5 personality, 7 significant correlation in 5 values. The personality model is mostly widely used model to describe how a person engages with the world. When people consider to purchase a car, comparing with their personality, their own values drive them to make the decision. That conscientiousness is negatively correlated with preference of safety ($p=0.02$) which means the conscientious people do not care the safety when they purchase a car. The conservative people tend to like safety ($p=0.002$), and do not care price ($p=0.002$). And for people who open to change, they do not care price ($p=0.04$), but they tend to like performance. The people who desire to self-enhance tend to like luxury car ($p<0.0001$). The people who desire to self transcend do not care about style ($p=0.001$), but concern about fuel economy ($p=0.002$).
\subsection{Pattern Discovery with Constrained Clustering} 
\input{tbl/tbl_cluster_pattern_new} 
%\begin{figure}
%	\centering
%    \includegraphics[width = 7.5cm]{img/feature_preference_level.jpg}
%    \caption{Distributions of Aspect Preferences}
%    \label{fig:level_perference}
%\end{figure}
In the regression analysis, we have only considered the main effects. In order to discover high-order interaction patterns with limited data, we used clustering to group people who share similar traits together. In addition, we also wanted the people within a cluster to share similar aspect preferences.  Otherwise, we won't be able to link the trait patterns discovered in a cluster with aspect preferences. Thus, we employed constrained clustering in this analysis. With constrained clustering, we can ensure the homogeneity of the aspect preferences within each resulting cluster. 
To facilitate this analysis, first we  mapped the aspect ranks obtained in Task 3 into discrete categories. Specifically,  for a complete rank of eight car aspects,  we mapped the top three ranked aspects to an ``Important" class, bottom three to a ``Not-Important" class, and the middle two to a ``Neutral" class. 
%Figure~\ref{fig:level_perference} shows the distribution of these categories for each car aspect. 
%Moreover, for constrained clustering, since it is a semi-supervised algorithm, we will use all the data collected in task 1, 2, and 3. In total, 1475 data points for training and 100 for testing. Among the 1475 training instances, 494 with car aspect preference labels and 981 only with personal traits information. 
In addition, we encoded the aspect homogeneity requirement as additional constraints. Typically, constrained clustering incorporates either a set of must-link constraints, cannot-link constraints, or both. Both a must-link and a cannot-link constraint define a relationship between two data instances. A must-link constraint is used to specify that the two instances in the must-link relation should be placed in the same cluster. A cannot-link constraint is used to specify that the two instances in the cannot-link relation should not be put in the same cluster. These constraints act as a guide for which a constrained clustering algorithm will use to find clusters that satisfy these constraints.  
To encode the homogeneity requirement, for each car aspect (e.g. car safety), we can simply add must-links between every pair of Turkers if they share the same aspect preference (e.g., both consider ``safety" important) and add cannot-links for every pair of Turkers who do not share the same aspect preferences (e.g., one Turker considers ``safety" ``Important", the other considers it ``Not-Important"). But this encoding is not ideal since with both must-links and cannot-links, it is very likely we will get three big clusters for each aspect, each is related to one of the three categories: Important, Neutral and Not-Important. Although the resulting clusters satisfy the homogeneity of the aspect preference requirement, they fail to group people with similar traits together. As a result, in this analysis, we only used cannot-links,  which not only guarantees the homogeneity of aspect preferences, but also creates smaller clusters that group people with similar traits together. 
We employed the Metric Pairwise Constrained KMeans algorithm (MPCK-MEANS)~\cite{bilenko2004integrating} to incorporate the aspect preference homogeneity requirement.  The optimal cluster number $K$ for each aspect was determined empirically by running MPCK-MEANS with different $K$s, $K\in[3,20]$  (3 is the minimum number of clusters since we have 3 different aspect preference categories).  
To determine whether the resulting clusters capture any significant patterns, we used two pattern selection criteria (a) a homogeneity criterion which requires that there is at least one trait whose values in the cluster is relatively homogeneous; (b) a distinctiveness criterion which requires that  for the traits identified in (a), their cluster means need to be significantly different from the population means.  For (a), we used the coefficient of variation (CV) as the homogeneity measure. CV, also known as relative standard deviation (RSD), is a standardized measure of dispersion of a probability or count distribution. It is often expressed as a percentage and is defined as the ratio of the standard deviation $\sigma$  to the mean $|\mu|$. In the study, we required that all the CVs of homogeneous traits to be lower than 0.12.  For (b) we required that the differences of the means need to be significant based on an independent sample t-test with $p<0.001$ and the difference of means is greater than 0.2. Table~\ref{tbl:pattern} highlights some of the patterns discovered using this approach. In this table, we list the cluster id,  cluster label (Important, Not-Important, Neutral), clustering accuracy, and significant traits in the cluster (``+" indicates that the cluster mean is higher than population mean, ``-" means the opposite). For example, based on the Safety-1 pattern, people who are more extraverted (extrave (+)) and more neurotic (neurotic (+)) tend to consider ``car safety" important.   Similarly, based on pattern Safety-3, people who are more conscientious (conscie(+)) but less open (open(-)) tend to consider ``safety" important. Other interesting patterns include: people who are less open (open(-)) and do not value hedonism (hedomis (-)) don't consider performance very important (performance-3), and people who are more extraverted (extrave(+)), value hedonism and self-enhancement (hedonis(+), self-en(+))  do not think durability important (durability-1). 
%For each feature, we establish ML constraints between instances with same preference in level 1 and level 3, and CL constraints between instances from different levels (level 1 and level 3). Since user in the level 2 do not have obvious tendency, we do not set any constraints and let metric distance to determine their tendency. To evaluate the results, we use 494 instances to train clusters, and other 100 instances to test the results. Table \ref{tbl:constraint} shows the number of the constraints generated from the training dataset for each feature. 
%In these regression models, there are ten independent variables, it is hard to consider all combination of interactions in regression, since it can be from 2-way to 10-way interactions. There are too many parameters relative to the number of observations. Fitting many interactions might lead to overfitting. However, due to decision making can be involved a variety of dimensions of a person, main effects are not sufficient to interpret the users' choice better. In order to investigate the effective interactions among different traits, we applied clustering analysis on the reader data, and extracted effective patterns for feature preference. 
%\begin{table}[h]
%\label{tbl:constraint}
%\caption{Number of constraints}
%\centering
%\begin{tabular}{|c|c|c|} \hline
%   & MLs & CLs \\ \hline
%Safety	&50151	&27664\\ \hline
%Fuel	&41796	&23545\\ \hline
%Quality	&30123	&25488\\ \hline
%Style	&50188	&26840\\ \hline
%Price	&61506	&13960\\ \hline
%Luxury	&98056	&7974\\ \hline
%Performance	&29071	&20384\\ \hline
%Durability	&24991	&24464\\ \hline
%\end{tabular}
%\end{table}
%Another problem is how to determine the number of clusters are appropriate for MPCK-Mean algorithm of our dataset. Since we concern the quality of clustering and also the constraints' satisfaction which help us to understand readers' preference within cluster. We therefore combined these two aspects together to measure the effectiveness of clustering. We measured the internal quality of clustering with cohesion and separation. Cohesion is represented how closely related are instances in a cluster which is measured by the within clusters sum of squares(SSE). Separation is represented how distinct a cluster is from other cluster which is measured by the between cluster sum of square(BSS)\cite{•}. Our basic procedure has the following steps for estimating the number of clusters:
%\begin{enumerate}
%\item Run the MPCK-Mean algorithm for different numbers of clusters, K is from 2 to 7 in our study.
%\item For different K, calculate the constraints satisfactions($C_{k}$): 
%\begin{align*}
%	C = \sum_{i}^{K} S_{i}
%\end{align*}
%$S_{i}$ is the number of satisfied constraints in the cluster. And then normalize $C$ with the total number of constraints:
%\begin{align*}
%	C ^{'} = \frac{\sum_{i} S_{i}}{ML + CL}.  
%\end{align*}
%$S_{i}$ is the number of constraints satisfied in the cluster.
%\item For different K, calculate $SSE$ and $BSS$:
%\begin{align*}
%WSS = \sum_{i}\sum_{x\in C_{i}} (x-m_{i})^2
%\end{align*}
%\begin{align*}
%BSS = \sum |C_{i}|(m-m_{i})^2,
%\end{align*}
%where $|C_{i}|$ is size of cluster i, m is the centroid of the whole data set. To get a straight-forward indicator of general quality of clustering, we normalize the sum of squares as:
%\begin{align*}
%SS^{'} = \frac{BSS}{BSS+WSS}.
%\end{align*}
%\item For different K, combine two indicators together as one indicator $r_{k}$ with $\alpha = 0.5$:
%\begin{align*}
%r = \alpha C^{'} + (1-\alpha)SS^{'}
%\end{align*}
%\item Find $k$ with maximum $r$.
%\end{enumerate}
%We find different optimal $k$ for different features showed in Table \ref{tbl:kValue}. The constraints attempted to group the items as two groups: level 1 (positive) and level 3 (negative). When $k$ equals to 2, the users of level 1 and the users of level 3 are completely separated. As $k$ is increased, positive group and negative group do not change internally, the algorithm split people with neutral attitude into one or more groups so that it does not impact on constraint satisfactions but impact on the internal quality of clustering. Such as for fuel,style,performance and durability, we get more than two sub-groups of users with neutral attitude. In our experiment, when $k$ is sometime greater than the actual number of clusters, because there are some empty clusters in results. 
%\begin{table}[h]
%\label{tbl:kValue}
%\caption{K value for different features}
%\centering
%\begin{tabular}{|l|c|c|} \hline
%Feature & $K$ & \thead{\# of \\clusters} \\ \hline
%Safety	&2&	2\\ \hline
%Fuel	&7&	5\\ \hline
%Quality	&2&	2\\ \hline
%Style	&7&	6\\ \hline
%Price	&3&	3\\ \hline
%Luxury	&3&	3\\ \hline
%Performance	&7&	7\\ \hline
%Durability	&6&	6\\ \hline
%\end{tabular}
%\end{table}
%To obtain the readers' profile in each cluster, we compare the users with our reference population. 
%Table 9-27 shows different readers' profiles for preference of different features. If we do not find any significant difference, that is to say no difference between the readers in the cluster and reference population. $Mean_{c}$ is mean of the normalized score of the trait in the cluster. $Diff$ shows the difference between the $Mean_{c}$ and mean in the reference population.  \begin{align}Diff = Mean_{c} - Mean_{general}.\end{align}
%When $Diff$ is greater than 0, it means the score of traits in the cluster is higher than the mean in general population, otherwise, it is lower than the mean.Table 9 shows the more agreeable and more self transcendent people tend to care about safety. And Table 10 shows less agreeable, less neurotic, less conservative and less self-transcendent people do not care about safety.There are three clusters for fuel economy, we do not find significant different in positive cluster. Table 12 shows the readers with higher score on extroversion, hedonism, open to change and self-enhancement do not care about fuel economy.  
%\input{tbl/tbl_safety_clustering}
%\input{tbl/tbl_fuel_clustering}
%\input{tbl/tbl_quality_clustering}
%\input{tbl/tbl_style_clustering}
%\input{tbl/tbl_price_clustering}
%\input{tbl/tbl_luxury_clustering}
%\input{tbl/tbl_performance_clustering}
%\input{tbl/tbl_durability_clustering}
%In the clusters of quality, table 16 there is one significant results found showed in table 16 which readers with lower score on hedonism rank the quality in the middle of position. Table 17 shows less open and less self transcendent people care about style. (neutral explanation)In the clusters of price, people with higher scores on consciousness, extroversion, conservation, hedonism, self-enhancement and self-transcendence do not care about price. In the clustering of luxury, people who are more self-enhancement care about luxury. As increasing the score of hedonism and decreasing the score of self-enhancement, people tend to neutral attitude to luxury.In the clustering of performance, people who are more hedonist, open to change and self-enhancement tend to like performance. (neutral) In the clustering of durability, people who are less hedonist tend to care about durability, and people who are self enhancement do not care about durability.
%\subsection {Building a Emphasis Framing Model}
%We also want to build a prediction model to verified if it is feasible to build a prediction model to determine which aspects to focus on based on a receiver's personal traits.
%We model this as a three-way classification task. For a given receiver's traits and a car aspect, we want to build a prediction model to determine whether this aspect is Important, Not-Important or Neutral to the receiver.
%In this experiment, we used SVM to build the classifier. We trained a SVM prediction model with the Radial Basis Function (RBF) Kernel. After parameter optimization, table~\ref{tbl:sum} shows the classification results. We compared the results with a majority-based baseline (always assigns a label based on the majority class).  
%After we map the ranks into three categories, we can model the decision of aspect selection as a classification problem. In addition to the data collected in Task3 which contain both a participant's aspect preferences and personal traits (594 Turkers), in order to take advantage of additional trait data collected in Task1 (836 Turkers) and Task2 (145 Turkers), we also employ constrained clustering, trying to discover distinctive trait patterns associated with distinct aspect preferences.
%Specifically, for classification, since it is a supervised learning task, the data used only include the 594 data points collected in Task 3.  We separated the data into two parts: 494 for training and 100 for testing. 


==> EMNLP2016 - arxiv/Introduction.tex <==
\section{Introduction}
Persuasion is an integral part of our personal and professional lives.  The topic of generating persuasive messages has been investigated in different fields with varied focuses. Psychologists focus on the cognitive, social and emotional processes of a persuader and a persuadee to understand what makes a communication persuasive \cite{hovland1953communication,petty1986elaboration,smith1996message}. Marketing researchers are interested in applying theories of persuasion in promoting consumer products \cite{szybillo1973resistance,han1994persuasion,campbell2000consumers,kirmani2004goal,ford2005speak,hirsh2012personalized}.   Natural Language Generation (NLG) researchers are interested in studying the relations between language usage and persuasion in order to build automated systems that produce persuasive messages \cite{guerini2011approaches,reiter2003lessons}.  

It is also generally believed that persuasion is more effective when it is custom-tailored to reflect the interests and concerns of the intended audience \cite{noar2007does,dijkstra2008psychology,hirsh2012personalized}.  A proven tailoring tactic  commonly used by politicians,  marketing executives, as well as public health advocators is content framing \cite{meyerowitz1987effect,maheswaran1990influence,grewal1994moderating,rothman1997shaping}.  Previous framing research has mainly focused on  two types of framing strategies: {\it emphasis frames} and {\it equivalence frames}. To {\it emphasis frame} a message is to simplify reality by focusing on a subset of the aspects of a situation or an issue and make them more salient in a communication  to promote certain definition, causal interpretation and moral evaluation~\cite{entman1993freezing}. For example, in political debating, {\it nuclear energy} can be framed as an {\it economic development} issue,  a {\it safety} issue or an  {\it environmental} issue.  In marketing, the same car can be framed as  a {\it low cost} car,  a {\it  performance} car, or a {\it green} car.  With different framing strategies, the authors try to appeal to individuals with different beliefs and concerns.  In contrast, {\it equivalence framing} focuses on presenting content as either loss-framed or gain-framed messages.  For example, a smoking cessation message can employ a gain-frame like  ``You will live longer if you quit smoking",  or a loss-frame such as ``You will die sooner if you do not quit smoking". Even though the messages are equivalent factually, the frames can influence a receiver's behavior either to encourage a desirable outcome or to avoid an outcome that is unwanted \cite{tversky1981framing}.

In this study, we focus on personalized {\it emphasis framing} which selects a subset of the aspects of an entity (e.g., a car) to enhance its appeal to a given receiver. In a car advertisement scenario, an emphasis framing model  decides which aspects of a car to emphasize to encourage certain user behaviors.  Thus, the communicative goal of emphasis framing is not to simply convey information, but to influence the opinion or behavior of a receiver.  

Using emphasis framing as the framework for personalized content selection, we can take advantage of rich findings in prior framing research that link content selection decisions to a set of psychologically-motivated domain-independent personal traits. This has made our work more generalizable than those relying on application-specific user characteristics (e.g.,  use an individual's smoking habit to tailor a smoke cessation message).   Since content framing is a part of  the content determination process, the model we propose is  a part of the {\it content planner} in a Natural Language Generation (NLG) system~\cite{reiter1997building}. 

There are three main contributions of this work. 

\begin{enumerate}
\item To the best of our knowledge, this is the first effort in building an automated model of emphasis framing for personalized persuasive message generation.
\item We made content selection decisions based on a set of psychologically-motivated application-independent user traits, such as  personality and basic human values, which makes our work more generalizable than the existing works that rely on domain-specific user characteristics and preferences.
\item We propose a cascade content selection model that integrates personalized content selection patterns uncovered in our analysis  in automated persuasive message generation. 
\end{enumerate}
 
%In the following, after a brief summary of related work, in Section 3, we  explain the personal trait models employed in the study.  To highlight the challenges in personalized emphasis framing, in Section 4, we describe an experiment to investigate whether non-expert humans are capable of performing emphasis framing effectively.  Section 5 presents a few experiments to analyze the relationship between a person's traits and his assessment of aspect importance.  We also propose a cascade content selection model to incorporate the study results in natural language generation.  Finally, in Section 7 we conclude this paper by summarizing the main findings.

%Organizational Behavior and Human Decision Processes Vol. 88, No. 1, May, pp. 411?429, 2002 A New Look at Framing Effects: Distribution of Effect Sizes, Individual Differences, and Independence of Types of Effects,  Irwin P. Levin, Gary J. Gaeth, Judy Schreiber, and Marco Lauriola.

%Much of the work on individual differences in persuasion has directly drawn on the persuasion theory of Elaboration Likelihood Model (ELM) (Petty and Cacioppo, 1986), a dual process model that explains how personal traits could moderate persuasion. Specifically, the ELM model states that there are two routes to persuasion: central and peripheral. The central route consists of thoughtful consideration of the arguments. The peripheral route occurs when the recipient decides whether to agree with the argument based on peripheral cues such as source credibility and attractiveness.  It also states that a person's likelihood to elaborate is determined by two things, a person's motivation and their ability to elaborate. 

%Previously, personalized content selection focus on tailoring the content based on topic interests, comprehension level, domain-specific user characteristics, 

%So far, very little is  known about exactly how to systematically frame the content of a message to enhance its personal appeal to a given individual.  The most common approaches for personalized persuasive message generation often apply hand-crafted rules to tailor content to domain-specific user characteristics.  

%General influence principles supported by social psychology and marketing research include {\it authority}, people are inclined to follow suggestions from authorities, {\it }

%While each of the influence principles described above has been shown to be effective and most have been used in the design of persuasive systems, the responses to these influence principles are not always clear-cut. For example, Johnson and Eagly(1989) discuss the difficulties many experimentals have had to replicate classical findings within the social influence field. These,and other, conflicting results are suggestive ofindividual differences in responses to influence principles.

%Nelson, T.E.; Clawson, R.A.; Oxley, Z.M. (1997). "Media framing of a civil liberties conflict and its effect on tolerance". American Political Science Review 91 (3): 567?583. 

%Research in the field of document design has demonstrate that content is one of important factor in determining the persuasiveness of a text(Hoeken 1995:). 

%In this paper, we present an comprehensive analysis to reveal how aspect message framing is influenced by personal traits. In our study, we focus on two types of personal traits: \textit{personality} and \textit{personal values}. \textit{Personality} refers to individual differences in mental, emotional, social and behavior characteristics; \textit{Personal value} reflects what is important to us and what motivates us in decision making. Thus, analyzing these personal traits may help us understand how to tailor message content to reflect the interests and concerns of the intended audience. In the first part of our study, we found personal traits have impact on aspect framing. To follow up on this finding, we compare the persuasive effectiveness between messages framed without consideration of audience personal traits versus message framed under consideration of these traits. Additionally, we collected people's traits and aspect selection data from the study, and used the data to train model to identify preference on feature selection. The results

%"System Personality and Persuasion in Human-Computer Dialogue" (PIERRE Y. ANDREWS TIIS 2012) explore how the personality of the user and the perceived personality of the system influence the user?s experience and the effectiveness of the persuasion. In the first experiment, we found that the users? extraversion significantly influences their perception of the dialogue and its persuasiveness. The second experiment provides more details on the perceived personality of the system and what influences such a perception; it also explores how trustworthiness and persuasiveness are shaped by the user experience during the dialogue. With these two exploratory experiments we have shown that the system?s generated personality can have an effect on its perception by the users and thus influence the actual persuasiveness output of the dialogue, even if the arguments presented are the same.

% Empirical Methods in Natural Language Generation Volume 5790 of the series Lecture Notes in Computer Science pp 242-263 "Towards Empirical Evaluation of Affective Tactical NLG" Ielka van der Sluis, Chris Mellish

%How to frame different persuasive messages for different customers is a challenge. In director marketing, can we tailor an advertisement to each consumer's characteristics to improve response rate? In health care, can we personalize each preventive care message such as cancer screening advice to induce more positive behavior changes? In marketing researches, it is common to categorize customers based on demographics such as age, gender, location and income. However, there are more existing individual differences among customers in same group, such as personality, personal values and individual needs, which mostly influence people's attitudes and economic decisions.

%Among them, the most influential theory of persuasion is the Elaboration Likelihood Model (ELM) (Petty and Cacioppo, 1986). It states that there are two ?routes? to persuasion: central and peripheral. The central route consists of thoughtful consideration of the arguments. The peripheral route occurs when the recipient decides whether to agree with the argument based on peripheral cues such as source credibility and attractiveness.  It also states that a person?s likelihood to elaborate is determined by two things, a person?s motivation and their ability to elaborate. Thus customizing the content and style of an argument based on a recipient?s motivation and ability can potentially enhance persuasion. 

%It is well-known that common expressions of probability have different meanings to different people. With any communication, but especially with persuasive communication, a understanding of the audience is critical. A thorough understanding of the target audience leads to insights into what the audiences' interests are and what potential objection they might have. A Framing message can be divided as two main questions: what to say and how to say. 

==> EMNLP2016 - arxiv/NLG.tex <==
 \section{Apply Emphasis Framing in NLG}
The patterns derived in the previous section can be used in personalized content selection for Natural Language Generation. In general, to promote a car, people tend to highlight the good aspects and avoid the bad aspects, regardless of a receiver's personality. For example, people will likely to highlight the fuel economy aspect  if a car is very fuel efficient while de-highlight the same aspect if a car is not fuel efficient. Thus, during content selection, to take the value of an aspect into consideration, we employ a cascade NLG model that integrates value-based content selection with trait-based personalization.  
The input to the cascade content selection model includes: (1) the values of all the aspects; (2) the trait scores of a given receiver; (3) the eight linear-regression models learned in Section 5.2, one for each aspect; (4)  the interaction rules learned in Section 5.3;  (5) n, the number of aspects needed in the output;  (6) the value difference threshold $\delta_1$ that determines whether the values of two or more aspects are significantly different; (7) the rank difference threshold $\delta_2$ that determines whether the ranks of two or more aspects predicted by the linear regression models are significantly different. To select n features to emphasize,  our system first ranks all the aspects based on their values. If the value of the  n-th aspect $v_n$ is significantly better than that of the (n+1)-th aspect $v_{n+1}$ (their difference is greater than $\delta_1$), we output the top n aspects directly.  Otherwise, for all the aspects whose values are either the same or not significantly worse than $v_n$, their ranks will be determined by the trait-based linear regression models. Moreover, after re-ranking relevant aspects based on the predicted ranks from the regression models, if the predicted rank of the n-th aspect ($r_n$) is significantly better than that of the (n+1)-th  aspect $r_{n+1}$ (the rank difference is greater than $\delta_2$), we just output the top n aspects in this list. Otherwise,  for those aspects whose ranks predicted by the linear regression models are not significantly lower than $r_n$, we use the interaction rules discovered in Section 5.3 to adjust their ranking scores (increase the rank by $\delta_2$ if ``Important", decrease by $\delta_2$ if ``Not-Important").  For each aspect, if more than one interaction rule applies, more accurate rules take precedence over less accurate rules.  Finally, the system will output top n aspects in the final list. Figure~\ref{fig:nlg} shows an example.  In this example, we assume n=3, $\delta_1$=1 and $\delta_2$=0.5. We first sorted all the aspects based on their values. Since the values of  ``Fuel Economy" and ``Luxury" are significantly better than the 3rd-ranked aspect ``Price",  their ranks are not affected by personalized aspect selection. Similarly, since the values of  ``Performance" and ``Style" are significantly lower than that of the 3rd-ranked aspect, their ranks are also not affected. Since the value differences among the rest 4 aspects, ``Price", ``Durability", ``Quality" and ``Safety" are all equal or not significant worse than $v_3$, we used trait-based personalized ranks from the regression models to re-rank them (the output ranks from the regression models are shown in the parentheses in the column ``Regression-based Re-Ranking").  After re-ranking these aspects based on the predicted ranks, since the rank of the 3rd-ranked aspect ``Price" (2.2) and that of ``Safety" (2.5) is within $\delta_2$, we use the learned interaction rules to adjust their ranks. Since the predicted ranks of ``Durability" and ``Quality" are much worse than  that of ``Price", their ranks are not affected by the interaction rules.  To apply the interaction rules, assume for a given receiver,  both his extraversion and neuroticism scores are much higher than the population average, the  Safety-1, Quality-1 and Performance-1 rules are applicable.  Since the Safety-1 rule predicts that  ``Safety" is ``Important" to the receiver while none of the rules affects ``Price",   the predicted rank for ``Safety" is increased by 0.5. After this adjustment, the ranks of all the aspects are shown in the ``Final Rank" column.  The top 3 aspects based on the final ranks are selected as the output (marked with a *).  
\begin{figure}
	\centering
	    \includegraphics[width = 7.5cm]{img/nlgexample.png}
 \caption{A Cascade Content Selection Example}
\label{fig:nlg}
\end{figure}

To evaluate the performance of the cascade content selection model, we conducted an additional AMT study.  Given the specifications of the ten cars in Task1, we asked  each AMT participant to select the top-n aspects to emphasize. Here n=1 and 3. In this task, aspect selection not only depends on the importance of an aspect to a receiver, but also the values of the aspects of a given car. We also acquired the personality and value scores of each Turker based on the IPIP personality and PVQ value survey. Finally, we compared the output of our model  with the aspects selected by the Turkers. We used top-n overlapping percentage as the evaluation metrics. Overall, we collected the aspect selection results from 38 Turkers, each on ten different cars. In total, we collected 380 data instances in our ground truth dataset.  We have tested different $\delta1$ and $\delta2$, the best results were obtained when $\delta1=0$ and $\delta2=0.5$. We compared our model with a baseline which purely relies on the values of aspects to determine their ranks. If two or more aspects have the same value (e.g., the values of both ``Price" and ``Durability" are ``3(Average)", their ranks were determined randomly. Table~\ref{tbl:nlgresults} shows the evaluation results, which demonstrate  a clear advantage of using the proposed cascade content-selection model. The Top-1 agreement is 62\% for the cascade model versus the baseline's 54\%. Similarly, if three aspects are needed in the output, the Top-3 agreement is 87\% versus the baseline's 46\%. All the differences are statistically significant based on the paired-t test ($p\leq0.05$).
%\begin{figure}[b]
%	\centering
	    %\includegraphics[width = 5.5cm]{img/nlgresults.png}
% \caption{Cascade Content Selection Evaluation}
%\label{fig:nlgresults}
%\end{figure}
\begin{table}[h]
\centering
\small
\caption{Cascade Content Selection Evaluation \label{tbl:nlgresults}}
\begin{tabular}{|c|c|c|} \hline
   &Cascade &Baseline\\ \hline
Top-1
agreement	&  0.62& 0.54\\ \hline
Top-3
agreement	&  0.87& 0.46\\ \hline
\end{tabular}
\end{table}
%In our previous analysis, we controlled the influence of aspect values (to keep all the aspect values unspecified).  Otherwise, the framing effect may be too subtle to detect, which is often the case when studying patterns related to human behaviors.  Thus,  the patterns we uncovered  in this study work only when the values of the input aspects are similar. To handle this, we propose a cascade content selection model to incorporate emphasis framing patterns in personalized content selection. 
%In a cascade content selection model, first a non-personalized, aspect value-based  content selection model is used. Based on  a preliminary study, selecting the aspect with the best value is a highly effective strategy.  When given a car with randomly generated values for all eight aspects, 91.4\% people selected the one with the best value. Moreover, if more customization is needed, we can employ the patterns learned in this study to select from aspects with similar values.  
%Figure~\ref{fig_task1} shows the distribution of selected aspect-values.
%\begin{figure}
%\centering
%\includegraphics[width = 7.5cm]{img/task1_task2_scale.jpg}
%\caption{The distribution of Selected Aspect Values}
%\label{fig_task1}
%\end{figure}
%In the following, we use an example to illustrate this process.  We were given the following car specification as input: safety: good, fuel economy: good, durability: ``bad". With the aspect value-based strategy, the system will  choose  the ``safety" and ``fuel economy" aspects,  but not the ``durability" aspect. In addition,  to choose between  ``safety" and ``fuel economy", both have a ``good" value, the system can emphasize the ``fuel economy" aspect (e.g.,  it is a green car)  to someone who values ``self-transcendent". However, framing it as a ``safe car" would be better if the receiver values ``conservation".

==> EMNLP2016 - arxiv/PreliminaryStudy.tex <==
\section{Acquiring Author Framing Strategy}
Framing effects are often subtle and may be influenced by many factors, such as the characteristics of the authors, the characteristics of the receivers and  the context of the communication. In the first study, we investigate whether it is feasible to build a personalized content selection model based on a writer's (a.k.a. an author's) content framing strategies. 
%To demonstrate the challenge, as a preliminary study, we investigate whether non-expert humans (authors)  are able to customize content for different individuals (receivers) effectively.  The results from this study have also motivated us to build content framing models based on a receiver's traits and preferences in instead of learning from the strategies used by non-expert authors.   

To investigate this, we first randomly generated ten cars, each include eight aspects: {\it safety, fuel economy, quality, style, price, luxury, performance and durability}.  The aspects were selected because similar features were used in prior automobile-related studies~\cite{Atkinson84,Beynon2001}. The value of each aspect was randomly generated on a 5-point Likert scale: ``1 (very bad)", ``2 (bad)", ``3 (average)", ``4 (good)", and ``5 (excellent)".  We also conducted a large-scale personality and basic human value survey on Amazon Mechanical Turk (AMT). We used the  50-item IPIP survey \cite{Goldberg:93} to obtain a Amazon Mechanical Turk worker (a.k.a. Turker)'s personality scores and the 21-item PVQ survey~\cite{schwartz:03} to obtain his/her basic value scores. To ensure the quality of the data from AMT, we added two qualification criteria.  A qualified Turker must  (1) have submitted over 5000 tasks  (2) with an acceptance rate over 95\%. The survey also included several validation questions. The validation questions are pairs of questions that are paraphrases of each other. If the answers to a pair of validation questions are significantly different, the user data were excluded from our analysis. After removing invalid data, we collected the traits of 836 Turkers.  Raw personality scores, ranging from 10 to 50, and raw value scores, ranging from 1 to 6, were computed directly from the survey answers.  The normalized trait scores, ranging from 0 to 1,  were computed using their rank percentiles in this population. 
%For example, a normalized score of 0.75 means its raw score ranks at 75\% in this population (or the raw score is higher than 25\% of the people in this population).

%\begin{table}[h]
%\centering
%\scriptsize
%\caption{An Example of Obtained Traits \label{tbl:persontrait}}

%\begin{tabular}{|c|c|c|c|} \hline
%  Model &Trait &RawS & NormalizedS\\ \hline
% Big& Agreeableness & 22 & 0.981\\ \cline{2-4}
%Five& Conscientiousness & 50 & 0.001\\ \cline{2-4}
%Person & Extraversion &  10 &  1.00\\ \cline{2-4}
%-ality & Neuroticisom & 12 & 0.988\\ \cline{2-4}
%  & openness & 40 & 0.45\\ \hline
%  & Conservation & 3.5 & 0.649\\ \cline{2-4}
 %Basic & Hedonism & 2.0 & 0.933\\ \cline{2-4}
% Human & Openness\_to\_change & 3.0 & 0.897\\ \cline{2-4}
% Values & Self\_Enhancement & 1.5 & 0.989 \\ \cline{2-4}
%  & Self\_Transcendence & 4.417 & 0.717\\ \hline
%\end{tabular}
%\end{table}
%
In addition, we designed two Human Intelligence Tasks (HITs) on AMT:  a content customization task and a validation task. In the content customization task (a.k.a. Task 1), a Turker was asked  to select one car aspect to emphasize in his campaign message for a receiver. The validation task (a.k.a. Task 2) was used to validate whether  a receiver prefers the message customized for her or not.

Specifically, in Task 1,  the Turkers were asked to imagine that they work for a marketing firm on a campaign to promote a new car. Each Turker was given the specification of a car ( randomly selected from the 10 randomly generated cars) and a receiver (randomly selected from the 836 Turkers whose trait scores were known to us).  The Turker was asked to write a campaign message to persuade the receiver to buy the car. But the Turker can only select one of the eight car aspects to include in his message. 
%Since customizing a message based on an interaction of all ten traits can be very challenging, we used a simplified trait profile in our study. The simplified trait profile contains only two traits:  the most prominent personality trait and the most prominent value trait.  The prominence of a trait was defined based on the normalized trait score.  The more different a trait score is from the median (.50), the more prominent the trait is. For example, for the Turker shown in table ~\ref{tbl:persontrait}, the most prominent personality and value traits are ``extraversion" and ``self-enhancement" (highlighted in bold face).  Based on the derived trait profile, the person shown in Table~\ref{tbl:persontrait} is a very introverted person (She has the lowest extraversion score which ranks at 100\% in this population) and does not value achievement and power that much (her self-enhancement score is very low, lower than 98.9\% people in this population).  
For comparison, for the same car, we also asked the same writer to select a car aspect for a different receiver who has an opposite trait profile. The opposite trait profile is defined as the one that is most dissimilar to the given trait profile (with the lowest cosine similarity) in our data.
 %(e.g., for the person shown in table~\ref{tbl:persontrait}, the receiver with the opposite trait profile is someone "very extraverted" and values ``self-enhancement" very much.).  
After the writer selected a car aspect, he also wrote a campaign message using the selected aspect.  Overall, after removing invalid data, we collected 490 pairs of messages for 131 pairs of receivers.  

To validate the framing effect, in Task 2,  we asked a new set of Turkers (receivers) to first complete an IPIP personality survey and a PVQ human value survey. Based on the survey results, we computed the trait profile for each of them. In addition, for each Turker (receiver) in Task 2,  we matched his/her trait profile with the 131 pairs of trait profiles collected in Task 1.  The profile with the highest matching score (computed based on cosine similarity) was selected and its associated message pair was also retrieved.

Then we presented the Turker with a pair of messages, one created for someone with matching trait profile, the other for someone with the opposite trait profile. We randomized the order of the messages.  Finally, we asked the Turker to rate which message they prefer more. If the framing strategies used by the Turkers (authors) in Task 1 were effective, then the Turkers (receivers) in Task 2 will prefer the messages tailored for them more than the ones tailored  for someone with the opposite trait profile.  Overall, after filtering out invalid data, we have collected the results from 145 Turkers.  
%Shimei: Specify the match criteria. What if there is no match.  Were they presented the messages or the features? 
Among the 145 Turkers (receivers) in Task 2, 77 of them prefer the messages written for them while 68  prefer the messages written for someone with the opposite traits. We performed a {\it sign test} to determine whether the difference is statistically significant and the result was negative ($p<0.2$).  

Although moderate personalization effects were found in previous framing research,  only expert-crafted messages were used~\cite{hirsh2012personalized}. Here, when Turkers (mostly non-experts) were asked to customize the messages based on a receiver's traits, no significant effects were found. In the next, since authors' emphasis framing strategies were not effective, we present several experiments designed to automatically derive emphasis framing strategies based on a receiver's traits and his/her aspect selection decisions. 
%The goal is to investigate how capable normal people are at customizing content to enhance a message's appealing to a given user. We performed three experiments on framing message on car sales. In our experiments, we randomly generated 10 cars, each car includes 8 features: safety, fuel economy, quality, style, price and cost, luxury, performance and durability. Each feature is rated on 5-point Likert scale in datasheet: very poor, poor, average, good and excellent. We also collected 836 people with their peronal traits' scores which would be our reference pupolation. \ref{table:tblTraits} shows personal traits considered in our study. The big 5 personality's scores are measured based on 50-item IPIP survey \cite{Goldberg:93}. The values' score are computed by using 21-item PVQ survey \cite{schwartz:03}. 
%\begin{table}[h]
%\caption{\label{font-table} Personal traits. }
%\begin{tabular}{|l|l|}
%\hline \bf Category & \bf Features  \\ \hline
%Personality(5) & \makecell[l]{ Aggreeableness \\ Conscientiousness \\Extraversion, Neuroticism \\ Openness}  \\
%\hline
%Values(5) &\makecell[l]{Conservation \\Hedonism \\Openness to change \\Self Enhancement\\ Self Transcendence }\\
%\hline
%\end{tabular}
%\label{table:tblTraits}
%\end{table}

%\begin{table}[h]
%\centering
%\caption{\label{font-table} Car: Datasheet.}
%\begin{tabular}{|l|l|}
%\hline \bf Feature & \bf Point  \\ \hline
%Safety & Excellent\\
%\hline
%Fuel Economy & Good\\
%\hline
%Quality & Poor\\
%\hline
%Style & Excellent\\
%\hline
%Price / Cost & Excellent\\
%\hline
%Luxury & Poor\\
%\hline
%Performance & Average\\
%\hline
%Durability & Average\\
%\hline
%\end{tabular}
%\label{table:tblTraits}
%\end{table}

%Task 1: Each participant is given a car datasheet, the datasheet is randomly selected from 10 cars. Each participant is asked to select one car feature in message. Then ask them to write a message to persuade people to purchase a new car. The recipient of a message is unspecified. In this task, we collect 500 messages.

%Task 2: Each participant is asked to compose a persuasive message of a given car for a specific reader. The reader is randomly selected from 836 people. Since there are 10 traits for each person, it is difficult for participant to compose their message based on all of them. In our study, we only provide a profile of a reader with most prominent personality and value. The prominence of a trait feature is computed based on its deviation from population mean. To express the prominent traits clearly, we represent the traits' value by using 5-point scale: Very Weak, Weak, Neutral, Strong and Very Strong, the rating is based on the trait score's ranking in the population. In this task, we collect 490 personalized messages for 131 different readers. Since we focus on two prominent traits, the scale of selected traits distribute on two sides: Very Weak, Weak and Strong, Very Strong. To investigate personal traits impacts on message framing, we create opposite versions of readers. For example, if there is a profile with Very Strong agreeableness and Conservation, the opposite version will be Very Weak agreeableness and Conservation. We generate new 131 readers with opposite traits and collect another 490 messages. 

%Task 3: Each participant is asked to answer survey questions to measure 10 personal traits, and show them two messages: one is written for the person who are most similar to him in task 2, another is written for the opposite one. In this task, we collect selection from 145 people. 

%The results from task 1 show feature selections are mostly driven by car feature value, writers tend to choose the feature with high values showed in Figure \ref{fig_task1}. We run chi-square test on feature selection data between task 1 and task 2 to see if the data is governed by the same distribution. We cannot accept the hypothesis with $p < 0.0001$. Most cars include more than one excellent or good features. One of car sheet shows the car includes two excellent(Quality, Price) and three good feature (Luxury, Performance, Durability). Without readers' profiles, 91\% writers focus on excellent features. After writers consider readers' profiles, 29\% writers tend to focus on good features especially luxury which make more attractive for those readers. In our car data, there is only one case which includes 2 good features and other features are very poor. We run chi-square test on feature selection for the car between task 1 and task 2, the $p = 1$ shows the data are consistent with a same distribution. We find when value of features are significantly different, the value is normally driven the selection decision, no matter whether the writer consider the reader's profile or not. 
%\begin{figure}
%	\centering
%    \includegraphics[width = 7.5cm]{img/task1_task2_scale.jpg}
%    \caption{The distribution of Feature selection in Task 1}
%    \label{fig_task1}
%\end{figure}

%We assumed if writers know more about recipient better, the message will be more persuasive. The results show 77 people prefer the message written for the similar people, and 68 people prefer the message written for opposite one. We perform sign test to determine whether there is biased towards the message matching to similar people. We did not see the significant result. And then we categorize readers based on 10 different traits, and run sign test on different subsets. Our results is showed in table \ref{table:tblSignedTest}, we only find the consciousness tend to choose matched massage with $p = 0.04$. For other categories, we did not find significant results, so we cannot conclude people prefer matched message. That means writers' judgments are normally different for the same person. For normal people, it is very challenging to infer the real needs of readers from personality and value. In next section, we focus on analyze how readers preferences are related to their trait.     

%\begin{table}[h]
%\caption{\label{font-table} Message Selection for people with difference traits (* $p < 0.05$)}
%\begin{tabular}{|l|c|c|}
%\hline Traits & \thead{\# \\ of people} & \thead{Similar \\(\%)} \\ \hline
%Agreeableness (+) & 28 & 57.1  \\ \hline
%Agreeableness (-) & 6 & 50  \\ \hline
%Conscientiousness (+)& 35 & 62.9  * \\ \hline
%Conscientiousness (-) &4& 75\\ \hline
%Extroversion (+) &2& 50 \\ \hline
%Extroversion (-) &16& 43.8\\ \hline
%Neuroticism (+)&17& 47.1\\ \hline
%Neuroticism (-)&12& 41.7\\ \hline
%Openness (+)&20& 50\\ \hline
%Openness (-)&5& 40\\ \hline
%Conservation (+)& 24&	70.8\\ \hline
%Conservation (-)& 7&	57.1\\ \hline
%Hedonism (+)	& 20&30\\ \hline
%Hedonism (-)	&15&53.3\\ \hline
%Openness to change	(+)&9	&66.7\\ \hline
%Openness to change	(-)	& 0&0\\ \hline
%Self enhancement	(+)	&10&50\\ \hline
%Self enhancement	(-)	&3&100\\ \hline
%Self transcendence	(+)	&52&51.9\\ \hline
%Self transcendence	(-)	&5&20\\ \hline
%\end{tabular}
%\begin{tablenotes}
%\small
%\item * $p < 0.05$
%\end{tablenotes}
%\label{table:tblSignedTest}
%\end{table}

==> EMNLP2016 - arxiv/RelatedWorks.tex <==
 \section{Related Work}
In the following, we summarize the research that is most relevant to our work including prior psychology and communication studies that link  emphasis framing with personal traits. Since  building computational models of emphasis framing was not the primary goal in these studies, we also include literature on personalized Natural Language Generation. 

\subsection{Emphasis Framing and Personal Traits}
There is a large body of social, marketing and communication theories on framing effects. Tversky and Kahneman \shortcite{tversky1981framing} state that human decisions are controlled partly by the formulation of the problem and partly by the norms, habits, and personal characteristics of the decision-maker. ~\cite{zaller1992nature,zaller1992simple} point out that framing essentially reorganizes information to increase accessibility of an issue dimension by highlighting one cognitive path that had previously been in the dark. Others argue that the framing effect is due to a change in the rank order of the values associated with different aspects through the interaction with the content found within a message \cite{nelson1997toward,chong2007framing,jacoby2000issue}. Although most research agrees that the characteristics of a receiver play an important role in framing effectiveness, there is a significant disagreement in what characteristics of a receiver result in framing effects.  For example, ~\cite{anderson2010framing} states that people with prior attitudes toward an issue can be influenced by frames, while Slothuus \cite{slothuus2008more} and Tabor et al. \cite{taber2009motivated} did not find a framing effect for those with strong values associated with the issue prior to exposure to the frame. The mixed results  may be due to the fact that many of these studies did not take into account that people with different traits  (e.g., different personality) may react to framing strategies differently.

Recently, personalized framing, especially personality-based framing research has become a hot topic. Among them, Hirsh~\shortcite{hirsh2012personalized} investigates whether a persuasive appeal's effectiveness can be increased by aligning message framing with a recipient's personality profile. In this study, for a given mobile phone, they constructed five advertisements, each designed to target one of the five major personality traits. Their results indicate that advertisements were evaluated more positively when they cohered with participants' personality. In a separate study, ~\cite{conroy2012maternal} found that certain personality traits, particularly openness, agreeableness, and conscientiousness mediate framing effects when participants were presented with different frames of political and health issues such as civil liberties, medical treatments, energy, affirmative action, and gun control. 

Inspired by the above research, we also employ psychologically-motivated trait models to capture individual characteristics. In addition to personality, we also incorporate basic human values since framing effects are linked to personal beliefs and motivations.  As a result,  we have significantly increased the scope of our study over prior research. Moreover,  unlike prior research where only messages hand-crafted by experts were used, we are interested in building computational models to automatically select a subset of the aspects based on personal traits. 

%Slothuus, R. 2008. ?More Than Weighting Cognitive Importance: A Dual-Process Model of Issue Framing Effects.? Political Psychology 29(1): 1-28.

%Tabor, C. S., D. Cann, and S. Kucsova. 2009. ?The Motivated Processing of Political Arguments.? Political Behavior 31: 137-55.

% Erison, C., M. Lodge, and C. S. Taber. 2007. ?The Role of Affect on How People Think and Reason about Political Events and Public Policy.? Paper presented at the 2007 Annual Meetings of International Society of Political Psychology, Portland, OR

%Personalized content framing is very challenging. Due to the complexity of human decision process, the effect of framing is subtle and often determined by a large number of factors (e.g.,  the speaker's credibility, the audience's  beliefs and values, the topic, and the writing style).  Although previous research in psychology and behavior science has shown that hand-crafted messages adapted by experts to align with the personality traits of intended audiences  can increase their impact moderately ~\cite{Levin 2002, Hirsch2012},  it is unclear how to automate the process to obtain the same benefits. So far, very little is known to us on how to automatically select a subset of the aspects  to emphasize in a message based on individual traits. This research is the first to bridge this gap.

%Two types of frames are generally discussed in the social and behavior science literature. These two types include ?emphasis? framing where there is significant differences in what is in a frame (see Druckman 2001b) and ?equivalency? frames where where are minimal differences between frames (see Druckman 2001a). In the following, we focus on emphasis framing since in our study we will present different content to different people via content selection.

%Erison, C., M. Lodge, and C. S. Taber. 2007. ?The Role of Affect on How People Think and Reason about Political Events and Public Policy.? Paper presented at the 2007 Annual Meetings of International Society of Political Psychology, Portland, OR.

%Personality Traits Moderate Attribute Framing Effects, Eyal Gamliel, Ada H. Zohar,  Hamutal Kreiner, Social Psychological and Personality Science July 2014 vol. 5 no. 5 584-592, 
%This research examined whether two personality traits, namely agreeableness and conscientiousness, moderate the effect of attribute framing on the perceived fairness of allocation criteria. Two experiments showed that attribute framing affected the perceived fairness of allocation criteria for participants who score high on these personality traits. In contrast, participants who score low on these personality traits were relatively immune to attribute framing effect. Critically, these personality traits did not moderate the effect of attribute framing on evaluations in a nondistributive justice scenario. These findings are consistent with the possibility that highly agreeable and highly conscientious people are more sensitive to social issues, and, consequently, are more susceptible to attribute framing in scenarios that involve distributive justice (attribute framing is a part of equivalence framing)

%A Psychology of Framing: The Effects of Personality on Susceptibility to Media Frames,  Meredith Conroy PhdThesis, UC Santa Barbara.

%Investigate the framing effects on individuals with different personality traits with six political issues: civil liberties, medical research and treatments, energy, affirmative action, and gun control. The results show  that certain personality traits, particularly openness, agreeableness, and conscientiousness mediate framing effects.  

%Framing Traits: The Role of Personality in Framing Effects, Kristen Diane Anderson, Master Thesis,  University of Nebraska - Lincoln
\subsection{Personalized NLG}
There is also a large body of work on personalized Natural Language Generation (NLG). For example, STOP is a Natural Language Generation (NLG) system that generates tailored smoking cessation letters based on responses to a four-page smoking questionnaire~\cite{reiter2003lessons}; PERSIVAL customizes the content of search summaries based on its relevance to a given patient's health record~\cite{mckeown2003leveraging};  MATCH is a multimodal dialogue system that tailors the content of its responses based on a user's restaurant preferences;  M-PIRO tailors the words and complexity of museum object descriptions for different audiences (e.g. adults, children, and experts); PERSONAGE~\cite{biewen2011new} and CRAG 2~\cite{gill2012perceptions} vary linguistic styles  to project intended personality in spoken utterances.  Among them, STOP, PERSIVAL and MATCH use domain-specific user models while  M-PIRO, PERSONAGE and GRAG2 employ domain independent user properties, such as expertise and personality. For PERSONAGE and GRAG2,  personality traits are mainly used to adapt linguistic styles. So far, there has not been much work focusing on using domain-independent user traits to automatically adapt message content to improve its persuasive appeal. 

% Lessons from a failure: Generating tailored smoking cessation letters, Ehud Reiter, Roma Robertson, Liesl M. Osman , Artificial Intelligence 144 (2003) 41?58

%STOP is a Natural Language Generation (NLG) system that generates short tailored smoking cessation letters, based on responses to a four-page smoking questionnaire. A clinical trial with 2553 smokers showed that STOP was not effective; that is, recipients of a non-tailored letter were as likely to stop smoking as recipients of a tailored letter. In this paper we describe the STOP system and clinical trial. Although it is rare for AI papers to present negative results, we believe that useful lessons can be learned from STOP. We also believe that the AI community as a whole could benefit from considering the issue of how, when, and why negative results should be reported; certainly a major difference between AI and more established fields such as medicine is that very few AI papers report negative results.

%The STOP clinical trial did not tell us why STOP failed. There are many possible reasons for the negative result, including:
%(1) Tailoring cannot have much effect in this kind of application. That is, if a smoker receives a letter from his/her doctor about smoking, then the content of the letter is only of secondary importance, what is most important is simply the fact of having received a communication from his/her doctor encouraging smoking cessation.
%(2) Tailoring could have an impact, but only if it was based on much more knowledge about the smoker?s circumstances than is available via a 4-page multiple choice questionnaire.
%(3) Tailoring based on a multiple-choice questionnaire can work, we just did not do it right in STOP, due to inappropriate NLG or KA techniques, and/or invalid theoretical models of behaviour change.
%(4) The STOP letters did in fact have an effect on some groups (such as heavy or discouraged smokers), but the clinical trial was too small to provide statistically significant evidence of this

%Plausible arguments can be made for all of the above possibilities. For example, we could argue for (1) on the basis that brief discussions about smoking with a doctor have about a 2\% success rate [17], and this may be an upper limit for the effectiveness of a brief letter from a doctor. If so, then letters cannot do much better that the 1.8\% increase in cessation rates produced by the STOP non-tailored letter. Or we could argue for (2) by noting that during a number of informal discussions with smokers about our project, many people commented that in-depth knowledge of their circumstances would lead to more effective tailoring. We could also argue for (3) because there clearly are many ways in which the tailored letters could have been improved; and for (4) on the basis of the weak evidence for this mentioned in Section 4.2.

% Speaking the users' languages A. Isard, J. Oberlander, C. Mathes, I. Androutsopoulos, IEEE Intelligent Systems  (Volume:18 ,  Issue: 1 ) Page(s): 40 - 45, 2003

%The authors describe a system that generates descriptions of museum objects tailored to the user. The texts presented to adults, children, and experts differ in several ways, from the choice of words used to the complexity of the sentence forms. M-PIRO can currently generate text in three languages: English, Greek, and Italian. The grammar resources are language independent as much as possible. M-PIRO's system architecture is significantly more modular than that of its predecessor ILEX. In particular, the linguistic resources, database, and user-modeling subsystems are now separate from the systems that perform the natural language generation and speech synthesis. 

% Leveraging a Common Representation for Personalized Search and Summarization in a Medical Digital Library, Kathleen R. McKeown Noemie Elhadad Vasileios Hatzivassiloglou, Proceeding JCDL '03 Proceedings of the 3rd ACM/IEEE-CS joint conference on Digital libraries, Pages 159-170 

%we present techniques to personalize the results of search, making use of the online patient record as a sophisticated, pre-existing user model. Our work in PERSIVAL, a medical digital library, includes methods for re-ranking the results of search to prioritize those that better match the patient record. It also generates summaries of the re-ranked results which highlight information that is relevant to the patient under  the physician?s care. We focus on the use of a common representation for the articles returned by search and the patient record which facilitates both the re-ranking and the summarization tasks.This common approach to both tasks has a strong positive effect on the ability to personalize information. 

%Generation and evaluation of user tailored responses in multimodal dialogue, M.A. Walker,  S.J. Whittakera, A. Stent, P. Maloor, J. Moore, M. Johnston, G. Vasireddy, Cognitive Science Volume 28, Issue 5, September?October 2004, Pages 811?840

%When people engage in conversation, they tailor their utterances to their conversational partners, whether these partners are other humans or computational systems. This tailoring, or adaptation to the partner takes place in all facets of human language use, and is based on a mental model or a user model of the conversational partner. Such adaptation has been shown to improve listeners? comprehension, their satisfaction with an interactive system, the efficiency with which they execute conversational tasks, and the likelihood of achieving higher level goals such as changing the listener?s beliefs and attitudes. We focus on one aspect of adaptation, namely the tailoring of the content of dialogue system utterances for the higher level processes of persuasion, argumentation and advice-giving. Our hypothesis is that algorithms that adapt content for these processes, according to a user model, will improve the usability, efficiency, and effectiveness of dialogue systems. We describe a multimodal dialogue system and algorithms for adaptive content selection based on multi-attribute decision theory. We demonstrate experimentally the improved efficacy of system responses through the use of user models to both tailor the content of system utterances and to manipulate their conciseness.

%Multi-attribute decision models are based on the claim that if anything is valued, it is valued for multiple reasons (Keeney & Raiffa, 1976). In the restaurant domain, this implies that a user?s preferred restaurants optimize tradeoffs among restaurant attributes. To define a model for the restaurant domain, we must determine these attributes and their relative importance for particular users. We use a standard procedure called SMARTER that has been shown to be a reliable and efficient way of eliciting multi-attribute decision models for particular users or user groups (Edwards & Hutton Barron, 1994). The first step of the standard SMARTER procedure is to determine the structure of a tree model of the objectives in the domain. In MATCH, the top-level objective is to select a good restaurant. User interviews and data collection along with an analysis of online restaurant databases indicated that six attributes contribute to this objective: the quantitative attributes food quality, cost, decor, and service; and the categorical attributes food type and neighborhood (Whittaker, Walker, & Moore, 2002). These attributes are structured into the one-level tree shown in Fig. 6. A more complex structure that grouped decor, neighborhood and serviceunder a higher level objective called ambiance was considered, but informal questioning of users suggested this structure was less intuitive (Whittaker et al., 2002). The structure is user-independent with user-dependent weights on the branches as explained below.We apply this structure to a database of approximately 1000 restaurants populated with information freely available from the web.Values for each of these attributes for each restaurant are stored in the database.

%Perceptions of Alignment and Personality in Generated Dialogue, Alastair J. Gill, Carsten Brockmann and Jon Oberlander, INLG 2012 Proceedings of the 7th International Natural Language Generation Conference, pages 40?48.
 
%Variation in language style can lead to different perceptions of the interaction, and different behaviour outcomes. Using the CRAG 2 language generation system we examine how accurately judges can perceive character personality from short, automatically generated dialogues, and how alignment (similarity between speakers) alters judge perceptions of the characters? relationship. Whilst personality perception of our dialogues is consistent with perceptions of human behaviour, we find that the introduction of alignment leads to negative perceptions of the dialogues and the interlocutors?relationship. A follow up evaluation study of the perceptions of different forms of alignment in the dialogues reveals that while similarity at polarity, topic and construction levels is viewed positively, similarity at the word level is regarded negatively. We discuss our findings in relation to the literature and in the context of dialogue systems.

%The core notion here is that of emotion. This is reflected in the definition of de Rosis and Grasso (2000) of Affective Natural Language Generation: nlg that relates to, arises from or deliberately influences emotions or other non-strictly rational aspects of the Hearer.

%In linguistics, a notion closely related to that of affect has gained some currency. The notion in question is that of stance. The term ?stance? is defined from the speaker?s perspective: In addition to communicating propositional content, speakers and writers commonly express personal feelings, attitudes, value judgements, or assessments; that is, they express a ?stance?. (Biber et al., 1999:966)

%Authoring and Generating Health-Education Documents That Are Tailored to the Needs of the Individual Patient, Graeme Hirst, Chrysanne DiMarco, Eduard Hovy, Kimberley Parsons, Chapter, User Modeling, Volume 383 of the series International Centre for Mechanical Sciences pp 107-118

%Health-education documents can be much more effective in achieving patient compliance if they are customized for individual readers. For this purpose, a medical record can be thought of as an extremely detailed user model of a reader of such a document. The HealthDoc project is developing methods for producing health-information and patient-education documents that are tailored to the individual personal and medical characteristics of the patients who receive them. Information from an on-line medical record or from a clinician will be used as the primary basis for deciding how best to fit the document to the patient. In this paper, we describe our research on three aspects of the project: the kinds of tailoring that are appropriate for health-education documents; the nature of a tailorable master document, and how it can be created; and the linguistic problems that arise when a tailored instance of the document is to be generated.

% Influencing Individually: Fusing Personalization and Persuasion, Shlomo Berkovsky, Jill Freyne, Harri Oinas-Kukkonen	(ed.), Journal ACM Transactions on Interactive Intelligent Systems (TiiS),  Volume 2 Issue 2, June 2012 , Article No. 9

%Personalized technologies aim to enhance user experience by taking into account users? interests, preferences, and other relevant information. Persuasive technologies aim to modify user attitudes, intentions, or behavior through computer-human dialogue and social influence. While both personalized and persuasive technologies influence user interaction and behavior, we posit that this influence could be significantly increased if the two technologies were combined to create personalized and persuasive systems. For example, the persuasive power of a one-size-fits-all persuasive intervention could be enhanced by considering the users being influenced and their susceptibility to the persuasion being offered. Likewise, personalized technologies could cash in on increased success, in terms of user satisfaction, revenue, and user experience, if their services used persuasive techniques. Hence, the coupling of personalization and persuasion has the potential to enhance the impact of both technologies. This new, developing area clearly offers mutual benefits to both research areas, as we illustrate in this special issue.

% [Mairesse and Walker2010] Franc?ois Mairesse and Marilyn, Walker. 2010. Towards personality-based user Personalized content selection, adaptation: Psychologically informed stylistic language generation. User Modeling and User-Adapted Interaction, 20(3):227?278

%Controlling User Perceptions of Linguistic Style: Trainable Generation of Personality Traits Francois Mairesse, Marilyn A. Walker, Computational Linguistics Volume 37, Number 3, 2011
 
%This paper describes PERSONAGE, a highly parameterizable language generator whose parameters are based on psychological findings about the linguistic reflexes of personality. We present a novel SNLG method which uses parameter estimation models trained on personality-annotated data to predict the generation decisions required to convey any combination of scalar values along the five main dimensions of personality. A human evaluation shows that parameter estimation models produce recognizable stylisticvariation along multiple dimensions, on a continuous scale, and without the computational cost incurred by over generation techniques.

% health-education material can be much more effective if it is customized for the individual patient in accordance with their medical conditions, demographic variables, personality profile, or other relevant factors. A recent special issue of Patient Education and Counseling (February 1999) reviewed key work in computer-generated tailoring of health information, including: smoking cessation (V.J. Strecher; W.F. Verlicer and J.O. Prochaska), nutrition (J. Brug et al.), and potential benefits of tailoring (D.S. Bental, A. Cawsey, and R. Jones; A. Dijkstra and H. De Vries).

%(DiMarco et al. 07) rely instead on the pre-authoring of a ?library? of reusable text, annotated with linguistic and formatting information, and a subsequent process of customization in which reader appropriate pieces of text are selected, assembled, and automatically revised by computational ?textrepair? experts

%Dimarco_07:  The Development of a Natural Language Generation System For Personalized e-Health Information
%C. DiMarcoa, H. Dominic Covveyb, P. Brayc, D. Cowana,d, V. DiCiccioa, E. Hovye, J. Lipac, D. Mulhollandd

%Equivelence Framing

%In message framing theory, communicators basically use two ways of presenting information; messages are presented in terms of either the gain or loss, depending on the information provider’s bias and intention regarding impact. A classic example of how framing impacts opinion and choice is an experiment by Kahneman and Tversky (1984) that monitored patients' decisions on whether or not to undergo a surgical procedure. The study revealed that people tend to more often agree to a surgery if risks are presented in terms of survival rates (as in, 94 percent survive this procedure) than death rates (6 out of a hundred people die from this procedure). Even if both outcomes are the same, people tend to make different choices based on how a scenario is framed.

%Aspect framing:
%More recently, a 2004 study conducted by Stanford University political science professors asked respondents if they support or oppose allowing an extremist group to hold a rally. When posed in terms of freedom of expression, the majority supported the group’s rights; if framed in terms of risk for violence, the majority opposed permitting the rally. Again, data shows that communicators can control public perception and decisions by strategically framing the messaging of an issue.

%n~\cite{Hirsch2012} In the current study, we extended this research to examine whether a persuasive appeal?s effectiveness can be increased by aligning the message framing with the recipient?s personality profile. For a single product, we constructed five advertisements, each designed to target one of the five major trait domains of human personality. In a sample of 324 survey respondents, advertisements were evaluated more positively the more they cohered with participants? dispositional motives. These results suggest that adapting persuasive messages to the personality traits of the target audience can be an effective way of increasing the messages? impact, and highlight the potential value of personality-based communication strategies.

%Computer-based personality judgments are more accurate than those made by humans \cite{Wu2015}: Judging others? personalities is an essential skill in successful social living, as personality is a key driver behind people?s interactions, behaviors, and emotions. Although accurate personality judgments stem from social-cognitive skills, developments in machine learning show that computer models can also make valid judgments. This study compares the accuracy of human and computer- based personality judgments, using a sample of 86,220 volunteers who completed a 100-item personality questionnaire. We show that (i) computer predictions based on a generic digital footprint (Facebook Likes) are more accurate (r = 0.56) than those made by the participants? Facebook friends using a personality questionnaire (r = 0.49); (ii) computer models show higher interjudge agreement; and (iii) computer personality judgments have higher external validity when predicting life outcomes such as substance use, political attitudes, and physical health; for some outcomes, they even outperform the self-rated personality scores. Computers outpacing humans in personality judgment presents significant opportunities and challenges in the areas of psychological assessment, marketing, and privacy


==> EMNLP2016 - arxiv/Traits.tex <==
 \section{Acquiring Personal Traits}
 \begin{figure}
	\centering
    \includegraphics[width=8cm]{img/traits.png}
    \caption{Description of Two Trait Models\label{fig:traits}}
\end{figure}
%\input{tbl/tbl_trait}
Since prior study often links framing effects to individual characteristics, such as personality and individual motivations and beliefs, here we focus on two widely-accepted trait models in psychology: the Big5 personality model~\cite{Goldberg:93} and Schwartz's basic human value model~\cite{schwartz:03}.  
%which is often used to explain the motivational bases of attitudes and behavior.  
Figure~\ref{fig:traits} shows the description of each of the Big5 personality traits along with each of the five basic human value traits.
 
To acquire the personality and value traits of a person, traditionally, psychometric tests, such as the IPIP test for Big 5 personality \cite{yarkoni2010abbreviation} and the PVQ survey for values ~\cite{schwartz:03}, were used.  Recent research in the field of psycholinguistics has shown that it is possible to automatically infer personal traits from one's linguistic footprint, such as tweets, Facebook posts and blogs \cite{yarkoni2010personality,celli2013relationships,chen2014understanding}.  Unlike psychometric tests, automated trait analysis allows us to infer personal traits for a large number of people, which makes it possible to scale up automated personal persuasion  for a very large population (e,g., millions of social media users).  
 
 %Goldberg, L. R. (1993). "The structure of phenotypic personality traits". American Psychologist 48 (1): 26?34.
 %Celli et al., 2013] Fabio Celli, Fabio Pianesi, David Stillwell, and Michal Kosinski. Workshop on computational personality recognition (shared task). In Proceedings of the Workshop on Computational Personality Recognition, 2013

==> EMNLP2016 - arxiv/tbl/ReaderUserDist.tex <==
\providecommand{\e}[1]{\ensuremath{\times 10^{#1}}}
\begin{table*}[ht!]
\label{tbl:ReaderUserDistP}
\centering
\begin{tabular}{|c|c|c|} \hline
Personality &Polarity& Number\\ \hline
\multirow{2}{*}{Agreeableness} & + & 114\\\hline
 & - & 121 \\ \hline
 \multirow{2}{*}{Conscientiousness} & + & 158\\\hline
 & - & 100 \\ \hline
 \multirow{2}{*}{Extroversion} & + & 83\\\hline
 & - & 132 \\ \hline
 \multirow{2}{*}{Neutoticism} & + & 186\\\hline
 & - & 93 \\ \hline
 \multirow{2}{*}{Openness} & + & 99\\\hline
 & - & 117 \\ \hline
\end{tabular}
\caption{Reader distribution based on personality}
\end{table*}

\providecommand{\e}[1]{\ensuremath{\times 10^{#1}}}
\begin{table*}[ht!]
\label{tbl:ReaderUserDistV}
\centering
\begin{tabular}{|c|c|c|} \hline
Value &Polarity& Number\\ \hline
\multirow{2}{*}{Conservation} & + & 131\\\hline
 & - & 77 \\ \hline
 \multirow{2}{*}{Hedonism} & + & 120\\\hline
 & - & 83 \\ \hline
 \multirow{2}{*}{Openness to change} & + & 113\\\hline
 & - & 117 \\ \hline
 \multirow{2}{*}{Self enhancement} & + & 122\\\hline
 & - & 105 \\ \hline
 \multirow{2}{*}{Self transcendence} & + & 104\\\hline
 & - & 120 \\ \hline
\end{tabular}
\caption{Reader distribution based on personality}
\end{table*}


==> EMNLP2016 - arxiv/tbl/safety_clustering.tex <==
\begin{table}[h]
\label{tbl:constraint}
\caption{Safety(-) Cluster}
\centering
\begin{tabular}{|c|c|c|c|c|} \hline
Traits & $Mean_{cluster}$ & Diff & $p-value$\\ \hline
Agreeableness&0.654&0.061&0.0001 **\\ \hline
Conscientiousness&0.737&0.017&0.12\\ \hline
Extraversion&0.528&0.015&0.27\\ \hline
Neuroticism	&0.686&0.035&0.02*\\ \hline
Openness&0.760&0.011&0.26\\ \hline
Conservation&0.576&0.036&0.008 *\\ \hline
Hedonism&0.601&-0.028&0.07\\ \hline
Openness_to_change&0.632&-0.017&0.13\\ \hline
Self_enhancement&0.571&-0.020&0.12\\ \hline
Self_transcendence&0.716&0.044&0.0002 **\\ \hline
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:constraint}
\caption{Safety(+) Cluster}
\centering
\begin{tabular}{|c|c|c|c|c|} \hline
Traits & $Mean_{cluster}$ & Diff & $p-value$\\ \hline
Agreeableness&0.747&-0.033&0.005 *\\ \hline
Conscientiousness&0.763&-0.009&0.31 \\ \hline
Extraversion&0.551&-0.008&0.46\\ \hline
Neuroticism&0.741&-0.019&	0.11\\ \hline
Openness&0.777&-0.006&0.44\\ \hline
Conservation&0.631&-0.019&0.06\\ \hline
Hedonism&	0.558&0.015&0.27\\ \hline
Openness_to_change&0.605&0.009&0.38\\ \hline
Self_enhancement&0.540&0.011&0.34\\ \hline
Self_transcendence&0.783&-0.024&0.008*\\ \hline

\end{tabular}
\end{table}

==> EMNLP2016 - arxiv/tbl/tbl__evaluation.tex <==
	Cascade	Baseline
"Top-1 
agreement"	0.623684211	0.547368421
"Top-3
agreement"	0.871929825	0.463157895


==> EMNLP2016 - arxiv/tbl/tbl__regression_evaluation.tex <==
\begin{table}[h]
\label{tbl:fuel_pos}
\caption{Fuel(+)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
	&SST	&SSE	&R^2 \\ \hline
Safety	&435.79	&425.25	&0.02\\ \hline
Fuel	&296.51	&302.18	&-0.02\\ \hline
Quality	&342.76	&340.47	&0.01\\ \hline
Style	&276.51	&300.32	&-0.09\\ \hline
Quality	&342.76	&340.47	&0.01\\ \hline
Price	&333.31	&335.38	&-0.01\\ \hline
Luxury	&186.75	&178.18	&0.05\\ \hline
Performance	&289.76	&342.77	&-0.18\\ \hline
Durability	&306.99	&311.41	&-0.01\\ \hline
\end{tabular}
\end{table}


==> EMNLP2016 - arxiv/tbl/tbl_cluster_pattern.tex <==
\providecommand{\e}[1]{\ensuremath{\times 8^{#1}}}
\begin{table*}[ht!]
\label{tbl:pattern}
\caption{Patterns in clusters for different features}
\centering
\begin{tabular}{|l|c|l|l|} \hline
Feature & Cluster \#.& Label & Significant traits \\\hline
%Safety
\multirow{5}{*}{Safety} 
&4&1&Self-en(+), Self-tr(+)\\\cline{2-4}
&7&-1&Neuroti(+), Open(+), Self-tr(+)\\\cline{2-4}
&11&0&Conscie(+), Open(-)\\\cline{2-4}
&12&0&Extrave(+), Open(-), Self-en(-)\\\cline{2-4}
&13&0&Openness(+), Open(+), Self-en(+)\\\hline


\multirow{3}{*}{Fuel}
&3&1&Agreeab(+), Hedonis(+)\\\cline{2-4}
&4&-1&Agreeab(-), Conscie(+), Self-en(+)\\\cline{2-4}
&8&1&Conscie(+), Extrave(+), Hedonis(-)\\\hline

\multirow{9}{*}{Quality}
&2&0&Neuroti(+), Open(+), Self-en(+), Self-tr(+)\\\cline{2-4}
&4&0&Neuroti(+), Open(-)\\\cline{2-4}
&5&-1&Conscie(+), Neuroti(+)\\\cline{2-4}
&9&0&Agreeab(-), Open(-)\\\cline{2-4}
&10&1&Conscie(+), Extrave(+)\\\cline{2-4}
&12&0&Hedonis(-), Open(-)\\\cline{2-4}
&13&-1&Agreeab(+), Extrave(+), Self-tr(+)\\\cline{2-4}
&14&1&Conscie(+), Openness(+)\\\cline{2-4}
&16&-1&Conserv(-), Hedonis(+), Self-tr(-)\\\hline


\multirow{3}{*}{Style}
&8&-1&Extrave(+), Self-tr(+)\\\cline{2-4}
&13&0&Conscie(+), Self-en(+)\\\cline{2-4}
&15&-1&Openness(+), Conserv(+)\\\hline

Price&1&-1&Neuroti(+), Open(+), Self-en(+)\\\hline


\multirow{6}{*}{Performance}
&1&0&Hedonis(-), Self-tr(-)\\\cline{2-4}
&2&0&Conserv(-), Self-en(-)\\\cline{2-4}
&8&-1&Extrave(+), Conserv(+)\\\cline{2-4}
&10&0&Neuroti(+), Openness(+)\\\cline{2-4}
&12&-1&Extrave(+), Openness(-), Open(-), Self-tr(-)\\\cline{2-4}
&17&-1&Conscie(+), Hedonis(-), Open(-), Self-en(-)\\\hline

\multirow{6}{*}{Durability}
&1&1&Agreeab(-), Conserv(-), Self-en(-)\\\cline{2-4}
&2&0&Conscie(+), Openness(+)\\\cline{2-4}
&7&-1&Extrave(+), Openness(+)\\\cline{2-4}
&10&-1&Neuroti(+), Self-en(+)\\\cline{2-4}
&13&1&Agreeab(+), Neuroti(+)\\\cline{2-4}
&14&0&Agreeab(+), Conscie(+), Open(-), Self-en(-)\\\hline
\end{tabular}
\begin{tablenotes}
\small
\item * label: 1 positive 0 neutral -1 negative
\end{tablenotes}
\end{table*}

==> EMNLP2016 - arxiv/tbl/tbl_cluster_pattern_2.tex <==
\providecommand{\e}[1]{\ensuremath{\times 8^{#1}}}
\begin{table*}[ht!]
\label{tbl:pattern}
\caption{Patterns in clusters for different features}
\centering
\begin{tabular}{|l|c|l|l|} \hline
Feature & Cluster \#.& Label & Significant traits \\\hline
%Safety
\multirow{7}{*}{Safety} 
&4&pos&Self-en(+), Self-tr(+)\\\cline{2-4}
&6&pos&Agreeab(+)\\\cline{2-4}
&7&neg&Neuroti(+), Open(+), Self-tr(+)\\\cline{2-4}
&9&pos&Open(-)\\\cline{2-4}
&11&neu&Conscie(+), Open(-)\\\cline{2-4}
&12&neu&Extrave(+), Open(-), Self-en(-)\\\cline{2-4}
&13&neu&Openness(+), Open(+), Self-en(+)\\\cline{2-4}
&14&pos&Hedonis(-)\hline


\multirow{3}{*}{Fuel}
&0&neu&Conserv(+)\\\cline{2-4}
&3&pos&Agreeab(+), Hedonis(+)\\\cline{2-4}
&4&neg&Agreeab(-), Conscie(+), Self-en(+)\\\cline{2-4}
&8&pos&Conscie(+), Extrave(+), Hedonis(-)\hline

\multirow{9}{*}{Quality}
&0&pos&Openness(+)\\\cline{2-4}
&1&pos&Self-en(-)\\\cline{2-4}
&2&neu&Neuroti(+), Open(+), Self-en(+), Self-tr(+)\\\cline{2-4}
&4&neu&Neuroti(+), Open(-)\\\cline{2-4}
&5&neg&Conscie(+), Neuroti(+)\\\cline{2-4}
&9&neu&Agreeab(-), Open(-)\\\cline{2-4}
&10&pos&Conscie(+), Extrave(+)\\\cline{2-4}
&11&pos&Openness(+)\\\cline{2-4}
&12&neu&Hedonis(-), Open(-)\\\cline{2-4}
&13&neg&Agreeab(+), Extrave(+), Self-tr(+)\\\cline{2-4}
&14&pos&Conscie(+), Openness(+)\\\cline{2-4}
&15&neg&Neuroti(+)\\\cline{2-4}
&16&neg&Conserv(-), Hedonis(+), Self-tr(-)\hline


\multirow{3}{*}{Style}
&3&neg&Self-en(+)\\\cline{2-4}
&4&neu&Neuroti(+)\\\cline{2-4}
&7&pos&Conscie(+)\\\cline{2-4}
&8&neg&Extrave(+), Self-tr(+)\\\cline{2-4}
&11&neu&Conserv(+)\\\cline{2-4}
&12&neg&Conscie(+)\\\cline{2-4}
&13&neu&Conscie(+), Self-en(+)\\\cline{2-4}
&14&pos&Self-en(-)\\\cline{2-4}
&15&neg&Openness(+), Conserv(+)\\\cline{2-4}
&16&pos&Self-en(+)\hline

Price&1&neg&Neuroti(+), Open(+), Self-en(+)\hline
Luxury&1&neu&Self-en(+)\hline

\multirow{6}{*}{Performance}
&0&neu&Self-tr(+)\\\cline{2-4}
&1&neu&Hedonis(-), Self-tr(-)\\\cline{2-4}
&2&neu&Conserv(-), Self-en(-)\\\cline{2-4}
&4&neg&Conscie(+)\\\cline{2-4}
&5&neg&Conscie(-)\\\cline{2-4}
&8&neg&Extrave(+), Conserv(+)\\\cline{2-4}
&9&neg&Agreeab(-)\\\cline{2-4}
&10&neu&Neuroti(+), Openness(+)\\\cline{2-4}
&11&pos&Hedonis(-)\\\cline{2-4}
&12&neg&Extrave(+), Openness(-), Open(-), Self-tr(-)\\\cline{2-4}
&15&neu&Openness(+)\\\cline{2-4}
&17&neg&Conscie(+), Hedonis(-), Open(-), Self-en(-)\hline

\multirow{6}{*}{Durability}
&0&pos&Openness(+)\\\cline{2-4}
&1&pos&Agreeab(-), Conserv(-), Self-en(-)\\\cline{2-4}
&2&neu&Conscie(+), Openness(+)\\\cline{2-4}
&4&pos&Open(-)\\\cline{2-4}
&6&neg&Openness(+)\\\cline{2-4}
&7&neg&Extrave(+), Openness(+)\\\cline{2-4}
&8&neg&Self-tr(+)\\\cline{2-4}
&9&neu&Self-tr(-)\\\cline{2-4}
&10&neg&Neuroti(+), Self-en(+)\\\cline{2-4}
&11&pos&Neuroti(+)\\\cline{2-4}
&13&pos&Agreeab(+), Neuroti(+)\\\cline{2-4}
&14&neu&Agreeab(+), Conscie(+), Open(-), Self-en(-)\\\cline{2-4}
&15&pos&Hedonis(-)\\\cline{2-4}
&16&neu&Self-en(+)\hline
\end{tabular}
\begin{tablenotes}
\small
\item * label: 1 positive 0 neutral -1 negative
\end{tablenotes}
\end{table*}

==> EMNLP2016 - arxiv/tbl/tbl_cluster_pattern_new.tex <==
\providecommand{\e}[1]{\ensuremath{\times 10^{#1}}}
\begin{table*}[ht!]
%\centering
\captionsetup{font=small}
\caption{Patterns Discovered in Clustering Analysis \label{tbl:pattern}}
%\scriptsize
\makebox[\linewidth]{
	\scriptsize
	\begin{tabular}{|c|c|c|c|l|} \hline
	Feature & Cluster & Accuracy & Label & Significant traits \\\hline
	\multirow{3}{*}{Safety} 
	%&6& 0.7 &pos&Hedonis(+),Open(+)\\\cline{2-5}
	%&8&0.7 &pos&Hedonis(-),Open(-)\\\cline{2-5}
	&1&0.7 &Important&Extrave(+),Neuroti(+)\\\cline{2-5}
	&2& 0.64&Neutral&Conscie(+),Hedonis(+),Open(+),Self-en(+)\\\cline{2-5}
	&3& 0.71&Important&Conscie(+),Open(-)\\\hline

	\multirow{2}{*}{Fuel}
	&1&0.54 &Neutral&Open(-),Self-en(-)\\\cline{2-5}
	&2&0.54 &Not-Important&Hedonis(+),Open(+),Self-en(+)\\\hline

	\multirow{3}{*}{Quality} 
	&1&0.43&Important&Extrave(+),Neuroti(+)\\\cline{2-5}
	&2&0.45&Non-Important&Hedonis(+),Open(+),Self-en(+)\\\cline{2-5}
	%&14&0.37&pos&Conscie(+),Neuroti(+)\\\cline{2-5}
	&3&0.45&Not-Important&Conscie(+),Open(-)\\\hline

	\multirow{3}{*}{Style}
	&1&0.5&Not-Important&Hedonis(-),Open(-)\\\cline{2-5}
	%&7&0.37&pos&Hedonis(+),Self-en(+)\\\cline{2-5}
	&2&0.55&Neutral&Conscie(+),Extrave(+),Neuroti(+)\\\cline{2-5}
	&3&0.62&Neutral&Conscie(+),Hedonis(+),Open(+),Self-en(+)\\\cline{2-5}
	%&14&0.65&pos&Hedonis(-),Open(-),Self-en(-)\\\cline{2-5}
	&4&0.74&Not-Important&Conscie(+),Open(-)\\\hline

	%Price
	%Luxury
	\multirow{3}{*}{Performance}
	%&10&0.44&neu&Hedonis(+),Open(+)\\\cline{2-5}
	%&13&0.41&pos&Conscie(+),Conserv(+),Hedonis(+),Open(+),Self-en(+)\\\cline{2-5}
	&1&0.73&Neutral&Extrave(+),Neuroti(+)\\\cline{2-5}
	&2&0.5&Neutral&Conscie(+),Open(-)\\\cline{2-5}
	&3&0.4&Not-Important&Hedonis(-),Open(-)\\\hline

	\multirow{2}{*}{Durability} 
	&1&0.56&Not-Important&Extrave(+),Hedonis(+),Self-en(+)\\\cline{2-5}
	%&8&0.37&neg&Conscie(+),Neuroti(+),Open(-)\\\cline{2-5}
	%&10&0.43&neg&Conscie(+),Extrave(+),Neuroti(+)\\\cline{2-5}
	&2&0.36&Important&Conscie(+),Hedonis(+),Open(+),Self-en(+)\\\hline
	
	\multicolumn{5}{l}{%
  			\begin{minipage}{6.5cm}%
    		\tiny Note: $CV < 0.12$ $P < 0.001$ $Diff > 0.2 $%
  			\end{minipage}%
		}\\
	\end{tabular}
}

\end{table*}

==> EMNLP2016 - arxiv/tbl/tbl_clustering_results.tex <==
\providecommand{\e}[1]{\ensuremath{\times 8^{#1}}}
\begin{table*}[ht!]
\label{tbl:pattern}
\caption{Patterns in clusters for different features}
\centering
\begin{tabular}{|l|c|l|l|} \hline
Feature & Cluster \#.& Label & Significant traits \\\hline
%Safety
\multirow{5}{*}{Safety} 
&4&1&Self-en(+), Self-tr(+)\\\cline{2-4}
&7&-1&Neuroti(+), Open(+), Self-tr(+)\\\cline{2-4}
&11&0&Conscie(+), Open(-)\\\cline{2-4}
&12&0&Extrave(+), Open(-), Self-en(-)\\\cline{2-4}
&13&0&Openness(+), Open(+), Self-en(+)\\\hline


\multirow{3}{*}{Fuel}
&3&1&Agreeab(+), Hedonis(+)\\\cline{2-4}
&4&-1&Agreeab(-), Conscie(+), Self-en(+)\\\cline{2-4}
&8&1&Conscie(+), Extrave(+), Hedonis(-)\\\hline

\multirow{9}{*}{Quality}
&2&0&Neuroti(+), Open(+), Self-en(+), Self-tr(+)\\\cline{2-4}
&4&0&Neuroti(+), Open(-)\\\cline{2-4}
&5&-1&Conscie(+), Neuroti(+)\\\cline{2-4}
&9&0&Agreeab(-), Open(-)\\\cline{2-4}
&10&1&Conscie(+), Extrave(+)\\\cline{2-4}
&12&0&Hedonis(-), Open(-)\\\cline{2-4}
&13&-1&Agreeab(+), Extrave(+), Self-tr(+)\\\cline{2-4}
&14&1&Conscie(+), Openness(+)\\\cline{2-4}
&16&-1&Conserv(-), Hedonis(+), Self-tr(-)\\\hline


\multirow{3}{*}{Style}
&8&-1&Extrave(+), Self-tr(+)\\\cline{2-4}
&13&0&Conscie(+), Self-en(+)\\\cline{2-4}
&15&-1&Openness(+), Conserv(+)\\\hline

Price&1&-1&Neuroti(+), Open(+), Self-en(+)\\\hline


\multirow{6}{*}{Performance}
&1&0&Hedonis(-), Self-tr(-)\\\cline{2-4}
&2&0&Conserv(-), Self-en(-)\\\cline{2-4}
&8&-1&Extrave(+), Conserv(+)\\\cline{2-4}
&10&0&Neuroti(+), Openness(+)\\\cline{2-4}
&12&-1&Extrave(+), Openness(-), Open(-), Self-tr(-)\\\cline{2-4}
&17&-1&Conscie(+), Hedonis(-), Open(-), Self-en(-)\\\hline

\multirow{6}{*}{Durability}
&1&1&Agreeab(-), Conserv(-), Self-en(-)\\\cline{2-4}
&2&0&Conscie(+), Openness(+)\\\cline{2-4}
&7&-1&Extrave(+), Openness(+)\\\cline{2-4}
&10&-1&Neuroti(+), Self-en(+)\\\cline{2-4}
&13&1&Agreeab(+), Neuroti(+)\\\cline{2-4}
&14&0&Agreeab(+), Conscie(+), Open(-), Self-en(-)\\\hline
\end{tabular}
\end{table*}

==> EMNLP2016 - arxiv/tbl/tbl_constraints_all.tex <==
\begin{table}[h]
\label{tbl:constraint}
\caption{Number of constraints}
\centering
\begin{tabular}{|c|c|c|} \hline
   & MLs & CLs \\ \hline
Safety & 71844 & 39312 \\ \hline
Fuel &62481 & 33660   \\ \hline
Quality & 43002	&36001\\ \hline
Style & 75351	&37224\\ \hline
Price & 89959	&20256 \\ \hline
Luxury & 141477	&11704\\ \hline
Performance & 43621	&29532\\ \hline
Durability & 34902	&34476 \\\hline
\end{tabular}
\end{table}

==> EMNLP2016 - arxiv/tbl/tbl_constraints_split.tex <==
\begin{table}[h]
\label{tbl:constraint}
\caption{Number of constraints}
\centering
\begin{tabular}{|c|c|c|} \hline
   & MLs & CLs \\ \hline
Safety	&50151	&27664\\ \hline
Fuel	&41796	&23545\\ \hline
Quality	&30123	&25488\\ \hline
Style	&50188	&26840\\ \hline
Price	&61506	&13960\\ \hline
Luxury	&98056	&7974\\ \hline
Performance	&29071	&20384\\ \hline
Durability	&24991	&24464\\ \hline
\end{tabular}
\end{table}

==> EMNLP2016 - arxiv/tbl/tbl_durability_clustering.tex <==
\begin{table}[h]
\label{tbl:durability_pos}
\caption{Durability(+)}
\centering
\begin{tabular}{|l|c|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.70&	-0.018&	0.24\\ \hline
Consci.	&0.76&	0.001&	0.93\\ \hline
Extro.	&0.54&	-0.004&	0.79\\ \hline
Neuro.	&0.72&	-0.001&	0.97\\ \hline
Openn.	&0.76&	-0.007&	0.52\\ \hline
Conser.	&0.60&	-0.014&	0.34\\ \hline
Hedon.	&0.53&	-0.038&	0.028 *\\ \hline
Open.	&0.59&	-0.024&	0.07\\ \hline
Slf-en.	&0.53&	-0.026&	0.06\\ \hline
Slf-tr.	&0.74&	-0.020&	0.11\\ \hline
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:durability_neg}
\caption{Durability(-)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.72&	0.005&	0.73\\ \hline
Consci.	&0.77&	0.019&	0.09\\ \hline
Extro.	&0.55&	0.009&	0.49\\ \hline
Neuro.	&0.74&	0.014&	0.33\\ \hline
Openn.	&0.77&	0.0001&	0.97\\ \hline
Conser.	&0.62&	0.012&	0.37\\ \hline
Hedon.	&0.58&	0.004&	0.8\\ \hline
Open.	&0.61&	0.001&	0.96\\ \hline
Slf-en.	&0.58&	0.026&	0.04 *\\ \hline
Slf-tr.	&0.76&	-0.003&	0.77\\ \hline
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:durability_neu}
\caption{Durability(neutral)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.72&	0.009&	0.55\\ \hline
Consci.	&0.74&	-0.018&	0.11\\ \hline
Extro.	&0.54&	-0.006&	0.67\\ \hline
Neuro.	&0.71&	-0.013&	0.38\\ \hline
Openn.	&0.78&	0.005&	0.6\\ \hline
Conser.	&0.61&	0.0001&	0.99\\ \hline
Hedon.	&0.60&	0.025&	0.13\\ \hline
Open.	&0.63&	0.018&	0.16\\ \hline
Slf-en.	&0.55&	-0.004&	0.77\\ \hline
Slf-tr.	&0.78&	0.018&	0.09\\ \hline
\end{tabular}
\end{table}


==> EMNLP2016 - arxiv/tbl/tbl_fuel_clustering.tex <==
\begin{table}[h]
\label{tbl:fuel_pos}
\caption{Fuel(+)}
\centering
\begin{tabular}{|l|c|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.72&-0.004&0.77\\ \hline
Consci.&0.75&0.005&0.637\\ \hline
Extro.&0.54&0.007&0.517\\ \hline
Neuro.&0.72&0.002&0.897\\ \hline
Open.&0.77&-0.003&0.7\\ \hline
Conser.&0.61&0.007&0.55\\ \hline
Hedon.&0.57&0.005&0.71\\ \hline
Open&0.61&-0.001&0.9\\ \hline
Slf-en.&0.54&0.009&0.4	\\ \hline
Slf-tr.&0.77&-0.013&0.19	\\ \hline
\end{tabular}
\end{table}

\begin{table}[h]
\label{tbl:fuel_neg}
\caption{Fuel(-)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.70&-0.01&0.51	\\ \hline
Consci.&0.77&0.01&0.32	\\ \hline
Extro.&0.59&0.05&0.006	*\\ \hline
Neuro.&0.73&0.004&0.83	\\ \hline
Openn.&0.77&0.004&0.74	\\ \hline
Conser.&0.64&0.02&0.12	\\ \hline
Hedon.&0.66&0.09& $< 0.0001$	***\\ \hline
Open.&0.67&0.06& 0.0002	**\\ \hline
Slf-en.&0.63&0.08& $< 0.0001$ ***\\ \hline
Slf-tr.&0.74&-0.02&0.1\\ \hline
\end{tabular}
\end{table}

\begin{table}[h]
\label{tbl:fuel_neu}
\caption{Fuel(neutral)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.72&0.0013	&0.94	\\ \hline
Consci.&0.75&0	&1	\\ \hline
Extro.&0.52&-0.02	&0.15	\\ \hline
Neuro.&0.72	&0.0006	&0.97	\\ \hline
Open.&0.76&	-0.0113	&0.31	\\ \hline
Conser.&0.61&	-0.0047	&0.77	\\ \hline
Hedon.&0.50	&-0.07&	0.0003 **\\ \hline
Open.&0.56&	-0.06	&0.0001	**\\ \hline
Slf-en.&0.50	&-0.05	&0.0006	**\\ \hline
Slf-tr.&0.75	&-0.01	&0.38	\\ \hline
\end{tabular}
\end{table}

==> EMNLP2016 - arxiv/tbl/tbl_luxury_clustering.tex <==
\begin{table}[h]
\label{tbl:luxury_pos}
\caption{Luxury(+)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.67&	-0.045&	0.32\\ \hline	
Consci.	&0.78&	0.026&	0.35\\ \hline
Extro.	&0.60&	0.057&	0.14\\ \hline
Neuro.	&0.70&	-0.026&	0.5\\ \hline
Openn.	&0.75&	-0.025&	0.27\\ \hline	
Conser.	&0.67&	0.061&	0.17\\ \hline
Hedon.	&0.62&	0.045&	0.36\\ \hline	
Open.	&0.65&	0.040&	0.31\\ \hline	
Slf-en.	&0.68&	0.126&	0.006	*\\ \hline
Slf-tr.	&0.72&	-0.043&	0.3\\ \hline	
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:luxury_neg}
\caption{Luxury(-)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.72&	0.003&	0.80\\ \hline
Consci.&	0.75&	-0.001&	0.87\\ \hline
Extro.	&0.54&	-0.005&	0.64\\ \hline
Neuro.	&0.72&	-0.000&	0.99\\ \hline
Openn.	&0.77&	0.002&	0.81\\ \hline
Conser.	&0.61&	-0.001&	0.88\\ \hline
Hedon.	&0.56&	-0.009&	0.48\\ \hline
Open.&	0.61&	-0.004&	0.7\\ \hline
Slf-en.&	0.54&	-0.013&	0.2\\ \hline
Slf-tr.&	0.76&	0.004&	0.59\\ \hline
\end{tabular}
\end{table}



\begin{table}[h]
\label{tbl:luxury_neu}
\caption{Luxury(neutral)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&	0.70&	-0.012&	0.69\\ \hline
Consci.&	0.76&	0.003&	0.89\\ \hline	
Extro.&	0.57&	0.031&	0.21\\ \hline	
Neuro.	&0.74&	0.014&	0.65	\\ \hline
Openn.	&0.76&	-0.009&	0.64\\ \hline	
Conser.&	0.60&	-0.015&	0.57\\ \hline	
Hedon.	&0.66&	0.09&	0.01	*\\ \hline
Open.&0.64&	0.025&	0.38\\ \hline	
Slf-en.&	0.65&	0.099&	0.0008	*\\ \hline
Slf-tr.&	0.72&	-0.036&	0.1	\\ \hline
\end{tabular}
\end{table}

==> EMNLP2016 - arxiv/tbl/tbl_performance_clustering.tex <==
\begin{table}[h]
\label{tbl:performance_pos}
\caption{Performance(+)}
\centering
\begin{tabular}{|l|c|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&	0.69&	-0.027&	0.17	\\ \hline
Consci.&	0.78&	0.021&	0.15\\ \hline	
Extro.	&0.56&	0.017	&0.3	\\ \hline
Neuro.&	0.72&	-0.0001	&0.99\\ \hline	
Openn.	&0.77&	-0.002	&0.82	\\ \hline
Conser.	&0.62&	0.009	&0.62\\ \hline	
Hedon.	&0.63&	0.053&	0.01	*\\ \hline
Open.	&0.66&	0.049&	0.004 **\\ \hline
Slf-en.	&0.61&	0.056&	0.003 **\\ \hline
Slf-tr.	&0.75&	-0.012&	0.4532	\\ \hline
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:performance_neg}
\caption{Performance(-)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.72&	0.005&	0.66\\ \hline	
Consci.&	0.75&	-0.004&	0.64\\ \hline	
Extro.&	0.53&	-0.011&	0.33	\\ \hline
Neuro.&	0.72&	-0.004&	0.75\\ \hline	
Openn.&	0.77&	-0.004&	0.62	\\ \hline
Conser.&	0.60&	-0.009&	0.41\\ \hline	
Hedon.&	0.56&	-0.017&	0.23\\ \hline	
Open.&	0.59&	-0.022&	0.0513	\\ \hline
Slf-en.&	0.53&	-0.022&	0.0540\\ \hline	
Slf-tr.&	0.75&	-0.005&	0.5818\\ \hline	
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:performance_neu1}
\caption{Performance(neutral)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.58&	-0.13&	$<0.0001$ ***\\ \hline
Consci.	&0.69&	-0.067&	$<0.0001$ ***\\ \hline
Extro.	&0.48&	-0.063&	0.0005	**\\ \hline
Neuro.	&0.63&	-0.093&	$<0.0001$ ***\\ \hline
Openn.	&0.73&	-0.045&	0.0002	**\\ \hline
Conser.	&0.57&	-0.044&	0.008	*\\ \hline
Hedon.	&0.50&	-0.075&	0.0002	**\\ \hline
Open.	&0.54&	-0.076&	$<0.0001$ ***\\ \hline
Slf-en.	&0.51&	-0.043&	0.0059	*\\ \hline
Slf-tr.	&0.66&	-0.098&	$<0.0001$ ***\\ \hline
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:performance_neu2}
\caption{Performance(neutral)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.83&	0.11&		$<0.0001$ ***\\ \hline
Consci.	&0.80&	0.042&		0.002	**\\ \hline
Extro.	&0.60&	0.058&		0.0009	**\\ \hline
Neuro.	&0.80&	0.08&		$<0.0001$ ***\\ \hline
Openn.	&0.82&	0.047&		$<0.0001$ ***\\ \hline
Conser.	&0.66&	0.046&		0.005	*\\ \hline
Hedon.	&0.62&	0.05&		0.02	*\\ \hline
Open.	&0.68&	0.065&		$<0.0001$ ***\\ \hline
Slf-en.	&0.59&	0.035&		0.053	\\ \hline
Slf-tr.	&0.86&	0.097&		$<0.0001$ ***\\ \hline
\end{tabular}
\end{table}

==> EMNLP2016 - arxiv/tbl/tbl_price_clustering.tex <==
\begin{table}[h]
\label{tbl:price_pos}
\caption{Price(+)}
\centering
\begin{tabular}{|l|c|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.71&-0.002&0.88\\ \hline	
Consci.&0.75&-0.006&0.48\\ \hline	
Extro.&0.53&-0.008&0.46	\\ \hline
Neuro.&0.72&-0.005&0.7\\ \hline	
Openn.&0.77&-0.0001&0.96	\\ \hline
Conser.&0.60&-0.012&0.23	\\ \hline
Hedon.&0.57&-0.006&0.63	\\ \hline
Open.&0.61&-0.009&0.38\\ \hline	
Slf-en.&0.54&-0.008&0.43	\\ \hline
Slf-tr.&0.75&-0.007&0.46\\ \hline	
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:price_neg}
\caption{Price(-)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.72&	0.001&	0.95\\ \hline	
Consci.	&0.80&	0.048&	0.03 *\\ \hline
Extro.	&0.60&	0.054&	0.03 *\\ \hline
Neuro.	&0.76&	0.043&	0.13\\ \hline	
Openn.	&0.78&	0.007&	0.64\\ \hline	
Conser.	&0.69&	0.074&	0.005 *\\ \hline
Hedon.	&0.64	&0.068&	0.04 *\\ \hline
Open.	&0.69&	0.076&	0.004 **\\ \hline
Slf-en	&0.63&	0.079&	0.01 *\\ \hline
Slf-tr	&0.81&	0.048&	0.02 *\\ \hline
\end{tabular}
\end{table}

\begin{table}[h]
\label{tbl:price_neu}
\caption{Price(neutral)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.72&	0.005&	0.78\\ \hline
Consci.	&0.76&	0.002&	0.87\\ \hline
Extro.	&0.55&	0.006&	0.7\\ \hline
Neuro.	&0.72&	-0.002&	0.92\\ \hline
Openn.	&0.77&	-0.002&	0.87\\ \hline
Conser.	&0.62&	0.012&	0.49\\ \hline
Hedon.	&0.57	&-0.005&	0.79\\ \hline
Open.	&0.61&	-0.001&	0.97\\ \hline
Slf-en.	&0.55&	-0.003&	0.85\\ \hline
Slf-tr.	&0.76&	0.003&	0.82\\ \hline

\end{tabular}
\end{table}



==> EMNLP2016 - arxiv/tbl/tbl_quality_clustering.tex <==
\begin{table}[h]
\label{tbl:quality_pos}
\caption{Quality(+)}
\centering
\begin{tabular}{|l|c|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.71	&0.003&	0.8	\\ \hline
Consci.&0.75&	0.005&	0.61\\ \hline	
Extro.&0.55&	0.01&	0.4	\\ \hline
Neuro.&0.71&	-0.003&	0.8\\ \hline	
Openn.&0.77&	0.003&	0.66\\ \hline
Conser.&0.61&	0.003&	0.74\\ \hline	
Hedon.&0.59&	0.01&	0.24	\\ \hline
Open.&0.62&0.01&	0.22\\ \hline	
Slf-en&0.56&	0.01&	0.2\\ \hline	
Slf-tr&0.76&0.006&	0.5\\ \hline	
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:quality_neg}
\caption{Quality(-)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.71&-0.005&0.82\\ \hline
Consci.&0.74&-0.012&0.61\\ \hline
Extro.&0.55&0.002&0.40\\ \hline
Neuro.&0.72&0.003&0.80\\ \hline
Openn.&0.77&-0.008&0.66\\ \hline
Conser.&0.62&0.016&0.75\\ \hline
Hedon.&0.59&0.013&0.24\\ \hline
Open.&0.63&0.002&0.22\\ \hline
Slf-en.&0.55&-0.0008&0.2\\ \hline
Slf-tr.&0.75&-0.008&0.51\\ \hline
\end{tabular}
\end{table}

\begin{table}[h]
\label{tbl:quality_neu}
\caption{Quality(neutral)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.71&-0.0004&0.97\\ \hline	
Consci.&0.76&0.002&0.88\\ \hline	
Extro.&0.53&-0.015&0.27\\ \hline	
Neuro.&0.72&0.002&0.88\\ \hline	
Openn.&0.77&0.001&0.9\\ \hline	
Conser.&0.60&-0.017&0.22\\ \hline	
Hedon.&0.54&-0.033&0.04	*\\ \hline
Open.&0.59&-0.021&0.11\\ \hline	
Slf-en.&0.53&-0.02&0.15\\ \hline
Slf-tr&0.76&-0.003&0.79\\ \hline	
\end{tabular}
\end{table}

==> EMNLP2016 - arxiv/tbl/tbl_readerdist.tex <==
\begin{table}[h]
\label{tbl:readerdist}
\centering
\begin{tabular}{|c|c|c|} \hline
Traits &Polarity& Number\\ \hline
\multirow{2}{*}{Agreeableness} & + & 114\\ \cline{2-3}
 & - & 121 \\ \hline
 \multirow{2}{*}{Conscientiousness} & + & 158\\ \cline{2-3}
 & - & 100 \\ \hline
 \multirow{2}{*}{Extroversion} & + & 83\\ \cline{2-3}
 & - & 132 \\ \hline
 \multirow{2}{*}{Neutoticism} & + & 186\\ \cline{2-3}
 & - & 93 \\ \hline
 \multirow{2}{*}{Openness} & + & 99\\ \cline{2-3}
 & - & 117 \\ \hline
\multirow{2}{*}{Conservation} & + & 131\\ \cline{2-3}
 & - & 77 \\ \hline
 \multirow{2}{*}{Hedonism} & + & 120\\ \cline{2-3}
 & - & 83 \\ \hline
 \multirow{2}{*}{Openness to change} & + & 113\\ \cline{2-3}
 & - & 117 \\ \hline
 \multirow{2}{*}{Self enhancement} & + & 122\\ \cline{2-3}
 & - & 105 \\ \hline
 \multirow{2}{*}{Self transcendence} & + & 104\\ \cline{2-3}
 & - & 120 \\ \hline
\end{tabular}
\caption{The distribution of Reader based on different traits}
\end{table}


==> EMNLP2016 - arxiv/tbl/tbl_regression.tex <==
\providecommand{\e}[1]{\ensuremath{\times 10^{#1}}}
\begin{table*}[ht!]
\captionsetup{font=small}
	\caption{Results of the Regression Analysis \label{tbl:regression}}
%\scriptsize
%\centering
	\makebox[\linewidth]{
		\scriptsize 
		\begin{tabular}{|c|l|l|l|l|l|l|l|l|} \hline
 		&Safety& Fuel & Quality & Style & Price &Luxury & Perf & Durab\\\hline
		Agreeableness & 0.39 & -0.52  &-0.53  &0.54  &0.81 & 0.004& -0.62&-0.27\\\hline
		Conscientiousness & -1.75 *	& -0.31	&0.80  &0.29  &-0.01&0.27&0.83&-0.12\\\hline
		Extroversion	& 0.69&-0.71  &0.008  &-0.25&-0.37&0.48&-0.07&0.224\\\hline
		Neurotisim&1.08 &-0.01&-0.46  &-0.11  &-0.32&-0.07&0.18&-0.28\\\hline
		Openness&	1.59	&-0.05&0.01 &-0.99 &0.36&-0.53&-0.46&0.07	\\\hline
		Conservation&1.99 ** &-0.99 &-0.66&0.84&-1.72 ** &0.21&0.38&-0.03\\\hline
		Hedonism &1.47 & -0.15&-0.69&0.16&0.51&-0.06&-0.82&-0.43\\\hline
		Openness to change&-2.15&0.08&0.58&0.48&-1.99 *&-0.38&2.29*&1.07\\\hline
		Self-enhancement&-1.39&-1.12&0.58&0.47&-0.31&2.41 ***&0.77&-1.41\\\hline
		Self-transcendence&1.33&2.37 **&1.36&-2.47 **&-0.91&-1.01&-0.33&-0.32\\\hline
		\multicolumn{9}{l}{%
  			\begin{minipage}{6.5cm}%
    		\tiny Note: $p < 0.05$, ** $p < 0.005$, *** $p < 0.0001$%
  			\end{minipage}%
		}\\
		\end{tabular}
	}
\end{table*}

==> EMNLP2016 - arxiv/tbl/tbl_regression_evaluation.tex <==
\begin{table}[h]
\label{tbl:fuel_pos}
\caption{Fuel(+)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
	&SST	&SSE	&R^2 \\ \hline
Safety	&435.79	&425.25	&0.02\\ \hline
Fuel	&296.51	&302.18	&-0.02\\ \hline
Quality	&342.76	&340.47	&0.01\\ \hline
Style	&276.51	&300.32	&-0.09\\ \hline
Quality	&342.76	&340.47	&0.01\\ \hline
Price	&333.31	&335.38	&-0.01\\ \hline
Luxury	&186.75	&178.18	&0.05\\ \hline
Performance	&289.76	&342.77	&-0.18\\ \hline
Durability	&306.99	&311.41	&-0.01\\ \hline
\end{tabular}
\end{table}


==> EMNLP2016 - arxiv/tbl/tbl_regression_train.tex <==
\providecommand{\e}[1]{\ensuremath{\times 10^{#1}}}
\small
\begin{table*}[ht!]
\label{tbl:regression}
\caption{Results of the Regression Analysis}
\centering
\begin{tabular}{|c|l|l|l|l|l|l|l|l|} \hline
 &Safety& Fuel & Quality & Style & Price &Luxury & Perf & Durab\\\hline
Agreeableness		&0.32	&-0.78	&-0.51	&0.70	&0.84	&0.01	&-0.46	&-0.11\\\hline
Conscientiousness	&-1.16	&0.02	&0.67	&0.28	&-0.74	&0.27	&0.86	&-0.19\\\hline
Extraversion		&1.21	&-0.42	&0.28	&-0.37	&-0.58	&0.50	&-0.27	&-0.35\\\hline
Neuroticism			&0.97	&-0.09	&-0.59	&-0.25	&-0.23	&-0.19	&0.44	&-0.04\\\hline
Openness			&2.02*	&0.33	&-0.15	&-1.16	&0.34	&-0.75	&-0.61	&-0.02\\\hline
Conservation		&2.10*	&-0.98	&-0.11	&1.04	&-1.50*	&0.18	&-0.37	&-0.37\\\hline
Hedonism			&1.27	&0.10	&-0.44	&0.25	&0.30*	&0.02	&-0.91	&-0.60\\\hline
Openness to change	&-1.83	&-0.18	&0.66	&0.57	&-2.20	&-0.44	&2.28*	&1.15\\\hline
Self-enhancement	&-1.70	&-1.63*	&0.02	&0.23	&-0.03	&2.46***	&1.79*	&-1.15\\\hline
Self-transcendence	&1.34	&2.51*	&1.25	&-2.86**	&-0.67	&-1.13	&-0.15	&-0.28\\\hline
\end{tabular}
\begin{tablenotes}
\small
\item * $p < 0.05$, ** $p < 0.005$, *** $p < 0.0001$
\end{tablenotes}

\end{table*}

==> EMNLP2016 - arxiv/tbl/tbl_safety_clustering.tex <==
\begin{table}[h]
\label{tbl:safety_pos}
\caption{Safety(+)}
\centering
\begin{tabular}{|l|c|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.\footnotemark &0.747&0.033&0.005 *\\ \hline
Consci.\footnotemark &0.763&0.009&0.31 \\ \hline
Extro.\footnotemark &0.551&0.008&0.46\\ \hline
Neuro.\footnotemark &0.741&0.019&	0.11\\ \hline
Openn.\footnotemark &0.777&0.006&0.44\\ \hline
Conser.\footnotemark &0.631&0.019&0.06\\ \hline
Hedon.\footnotemark&0.558&-0.015&0.27\\ \hline
Open.\footnotemark &0.605&-0.009&0.38\\ \hline
Slf-en.\footnotemark &0.540&-0.011&0.34\\ \hline
Self-tr.\footnotemark &0.783&0.024&0.008*\\ \hline
\end{tabular}
\end{table}
\addtocounter{footnote}{-9}
\footnotetext{Agreeableness}
\addtocounter{footnote}{1}
\footnotetext{Conscientiousness}
\addtocounter{footnote}{1}
\footnotetext{Extroversion}
\addtocounter{footnote}{1}
\footnotetext{Neurotisim}
\addtocounter{footnote}{1}
\footnotetext{Openness}
\addtocounter{footnote}{1}
\footnotetext{Conservation} 
\addtocounter{footnote}{1}
\footnotetext{Hedonism}
\addtocounter{footnote}{1}
\footnotetext{Openness to change}
\addtocounter{footnote}{1}
\footnotetext{Self-enhancement}
\addtocounter{footnote}{1}
\footnotetext{Self-transcendence}

\begin{table}[h]
\label{tbl:safety_neg}
\caption{Safety(-)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.654&-0.061&0.0001 **\\ \hline
Consci.&0.737&-0.017&0.12\\ \hline
Extro.&0.528&-0.015&0.27\\ \hline
Neuro.	&0.686&-0.035&0.02*\\ \hline
Openn.&0.760&-0.011&0.26\\ \hline
Conser.&0.576&-0.036&0.008 *\\ \hline
Hedon.&0.601&0.028&0.07\\ \hline
Open.&0.632&0.017&0.13\\ \hline
Slf-en.&0.571&0.020&0.12\\ \hline
Slf-tr.&0.716&-0.044&0.0002 **\\ \hline
\end{tabular}
\end{table}

==> EMNLP2016 - arxiv/tbl/tbl_style_clustering.tex <==
\begin{table}[h]
\label{tbl:style_pos}
\caption{Style(+)}
\centering
\begin{tabular}{|l|c|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&	0.67&	-0.04&	0.07	\\ \hline
Consci.&	0.73&	-0.02&	0.2	\\ \hline
Extro.&	0.53&	-0.01&	0.57	\\ \hline
Neuro.&	0.70&	-0.016&	0.4	\\ \hline
Open.&	0.74&	-0.025&	0.04 *\\ \hline
Conser.&	0.62&	0.008&	0.61	\\ \hline
Hedon.&	0.61&	0.034&	0.15553	\\ \hline
Open.&	0.62&	0.002&	0.9	\\ \hline
Slf-en.&	0.57&	0.021&	0.27\\ \hline	
Slf-tr.&	0.72&	-0.043&	0.007 *\\ \hline
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:style_neg}
\caption{Style(-)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.72&	0.0066&	0.70	\\ \hline
Consci.&	0.75&	-0.005&	0.57\\ \hline	
Extro.	&0.54&	-0.003&	0.74\\ \hline	
Neuro.	&0.72&	-0.00002&	0.99\\ \hline	
Open.	&0.77&	0.003&	0.64\\ \hline
Conser.	&0.60&	-0.008	&0.4\\ \hline	
Hedon.	&0.56	&-0.016&	0.22	\\ \hline
Open.	&0.61&	-0.008&	0.39\\ \hline	
Slf-en.	&0.54&	-0.0143&	0.19\\ \hline	
Slf-tr.	&0.77&	0.01&	0.26\\ \hline	
\end{tabular}
\end{table}

\begin{table}[h]
\label{tbl:style_neu1}
\caption{Style(neutral 1)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.82	&0.11&	$<0.0001$	***\\ \hline	
Consci.	&0.85	&0.097&	$<0.0001$	***\\ \hline	
Extro.	&0.65	&0.111&	$<0.0001$	***\\ \hline	
Neuro.	&0.85	&0.123&	$<0.0001$	***\\ \hline	
Openn.	&0.82	&0.045&	0.0001	**\\ \hline	
Conser.	&0.70&	0.085&	0.001	**\\ \hline	
Hedon.	&0.64	&0.06&	0.013	*\\ \hline	
Open.	&0.69&	0.071&	0.001	**\\ \hline	
Slf-en.	&0.62&	0.065&	0.006	*\\ \hline	
Slf-tr.	&0.84&	0.078&	$<0.0001$	***\\ \hline	
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:style_neu2}
\caption{Style(neutral 2)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.65&	-0.065&	0.003	**\\ \hline
Consci.&	0.73&	-0.026&	0.08	\\ \hline
Extro.	&0.48&	-0.064&	0.001	**\\ \hline
Neuro.	&0.63&	-0.086&	0.0001	**\\ \hline
Openn.	&0.75&	-0.022&	0.12	\\ \hline
Conser.	&0.57&	-0.038&	0.05\\ \hline	
Hedon.	&0.56	&-0.014&	0.53	\\ \hline
Open.&	0.6	&-0.015&	0.41\\ \hline	
Slf-en.	&0.54&	-0.006&	0.72\\ \hline	
Slf-tr.	&0.7&	-0.064&	0.0008	**\\ \hline
\end{tabular}
\end{table}

==> EMNLP2016 - arxiv/tbl/tbl_svm_majority.tex <==
\begin{table}[h]
\label{tbl:constraint}
\caption{Number of constraints}
\centering
\begin{tabular}{|c|c|c|c|} \hline
&	Majority&	SVM&	p \\\hline
Safety&	61&	61&	0.53\\\hline
Fuel&	57&	58&	0.45\\\hline
Quality&	44&	47&	0.31\\\hline
Style&	63&	63&	0.53\\\hline
Price&	71&	71&	0.53\\\hline
Luxury&	90&	91&	0.41\\\hline
Performance&	46&	50&	0.24\\\hline
Durability&	37&	42&	0.18\\\hline
\end{tabular}
\end{table}

==> EMNLP2016 - arxiv/tbl/tbl_trait.tex <==
\providecommand{\e}[1]{\ensuremath{\times 8^{#1}}}
\begin{table}
\label{tbl:traits}
\caption{Description of Two Trait Models}
\scriptsize
\centering
\begin{tabular}{| p{1cm} | p{2cm} | p{4cm}|} \hline
Model & Feature & Description\\\hline
 & Openness to experience &  The degree of intellectual curiosity, creativity and a preference for novelty and variety a person has. \\\cline{2-3}
\multirow{5}{1cm}{Big5 Personality Model}& Conscientious &  A tendency to be organized and dependable, show self-discipline, act dutifully, aim for achievement, and prefer planned rather than spontaneous behavior. \\\cline{2-3}
& Extraversion &   Energy, positive emotions, surgency, assertiveness, sociability and the tendency to seek stimulation in the company of others, and talkativeness. \\\cline{2-3}
& Agreeableness &  A tendency to be compassionate and cooperative rather than suspicious and antagonistic towards others. \\\cline{2-3}
& Neuroticism &  The tendency to experience unpleasant emotions easily, such as anger, anxiety, depression, and vulnerability. \\\hline
& Openness to Change &  The desire for independence and new, novel, exciting and challenging experiences. \\\cline{2-3}
 \multirow{5}{1cm}{Schwartz's human basic values}& Self-Enhancement &  The pursuit of self-interests including social status, prestige, resources and personal success through demonstrating competence. \\\cline{2-3}
& Conservation &  Self-restriction and conform to tradition, social expectations and norms;  Pursue safety, harmony and stability; resist to change \\\cline{2-3}
& Hedonism &  Pursuit of pleasure and sensuous gratification for oneself. \\\cline{2-3}
& Self-transcendence &  Concern and pursue the enhancement and protection of the welfare and interests of others as well as the protection for nature. \\\hline
\end{tabular}
\end{table}

==> tbl/ReaderUserDist.tex <==
\providecommand{\e}[1]{\ensuremath{\times 10^{#1}}}
\begin{table*}[ht!]
\label{tbl:ReaderUserDistP}
\centering
\begin{tabular}{|c|c|c|} \hline
Personality &Polarity& Number\\ \hline
\multirow{2}{*}{Agreeableness} & + & 114\\\hline
 & - & 121 \\ \hline
 \multirow{2}{*}{Conscientiousness} & + & 158\\\hline
 & - & 100 \\ \hline
 \multirow{2}{*}{Extroversion} & + & 83\\\hline
 & - & 132 \\ \hline
 \multirow{2}{*}{Neutoticism} & + & 186\\\hline
 & - & 93 \\ \hline
 \multirow{2}{*}{Openness} & + & 99\\\hline
 & - & 117 \\ \hline
\end{tabular}
\caption{Reader distribution based on personality}
\end{table*}

\providecommand{\e}[1]{\ensuremath{\times 10^{#1}}}
\begin{table*}[ht!]
\label{tbl:ReaderUserDistV}
\centering
\begin{tabular}{|c|c|c|} \hline
Value &Polarity& Number\\ \hline
\multirow{2}{*}{Conservation} & + & 131\\\hline
 & - & 77 \\ \hline
 \multirow{2}{*}{Hedonism} & + & 120\\\hline
 & - & 83 \\ \hline
 \multirow{2}{*}{Openness to change} & + & 113\\\hline
 & - & 117 \\ \hline
 \multirow{2}{*}{Self enhancement} & + & 122\\\hline
 & - & 105 \\ \hline
 \multirow{2}{*}{Self transcendence} & + & 104\\\hline
 & - & 120 \\ \hline
\end{tabular}
\caption{Reader distribution based on personality}
\end{table*}


==> tbl/safety_clustering.tex <==
\begin{table}[h]
\label{tbl:constraint}
\caption{Safety(-) Cluster}
\centering
\begin{tabular}{|c|c|c|c|c|} \hline
Traits & $Mean_{cluster}$ & Diff & $p-value$\\ \hline
Agreeableness&0.654&0.061&0.0001 **\\ \hline
Conscientiousness&0.737&0.017&0.12\\ \hline
Extraversion&0.528&0.015&0.27\\ \hline
Neuroticism	&0.686&0.035&0.02*\\ \hline
Openness&0.760&0.011&0.26\\ \hline
Conservation&0.576&0.036&0.008 *\\ \hline
Hedonism&0.601&-0.028&0.07\\ \hline
Openness_to_change&0.632&-0.017&0.13\\ \hline
Self_enhancement&0.571&-0.020&0.12\\ \hline
Self_transcendence&0.716&0.044&0.0002 **\\ \hline
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:constraint}
\caption{Safety(+) Cluster}
\centering
\begin{tabular}{|c|c|c|c|c|} \hline
Traits & $Mean_{cluster}$ & Diff & $p-value$\\ \hline
Agreeableness&0.747&-0.033&0.005 *\\ \hline
Conscientiousness&0.763&-0.009&0.31 \\ \hline
Extraversion&0.551&-0.008&0.46\\ \hline
Neuroticism&0.741&-0.019&	0.11\\ \hline
Openness&0.777&-0.006&0.44\\ \hline
Conservation&0.631&-0.019&0.06\\ \hline
Hedonism&	0.558&0.015&0.27\\ \hline
Openness_to_change&0.605&0.009&0.38\\ \hline
Self_enhancement&0.540&0.011&0.34\\ \hline
Self_transcendence&0.783&-0.024&0.008*\\ \hline

\end{tabular}
\end{table}

==> tbl/tbl__evaluation.tex <==
	Cascade	Baseline
"Top-1 
agreement"	0.623684211	0.547368421
"Top-3
agreement"	0.871929825	0.463157895


==> tbl/tbl__regression_evaluation.tex <==
\begin{table}[h]
\label{tbl:fuel_pos}
\caption{Fuel(+)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
	&SST	&SSE	&R^2 \\ \hline
Safety	&435.79	&425.25	&0.02\\ \hline
Fuel	&296.51	&302.18	&-0.02\\ \hline
Quality	&342.76	&340.47	&0.01\\ \hline
Style	&276.51	&300.32	&-0.09\\ \hline
Quality	&342.76	&340.47	&0.01\\ \hline
Price	&333.31	&335.38	&-0.01\\ \hline
Luxury	&186.75	&178.18	&0.05\\ \hline
Performance	&289.76	&342.77	&-0.18\\ \hline
Durability	&306.99	&311.41	&-0.01\\ \hline
\end{tabular}
\end{table}


==> tbl/tbl_cluster_pattern.tex <==
\providecommand{\e}[1]{\ensuremath{\times 8^{#1}}}
\begin{table*}[ht!]
\label{tbl:pattern}
\caption{Patterns in clusters for different features}
\centering
\begin{tabular}{|l|c|l|l|} \hline
Feature & Cluster \#.& Label & Significant traits \\\hline
%Safety
\multirow{5}{*}{Safety} 
&4&1&Self-en(+), Self-tr(+)\\\cline{2-4}
&7&-1&Neuroti(+), Open(+), Self-tr(+)\\\cline{2-4}
&11&0&Conscie(+), Open(-)\\\cline{2-4}
&12&0&Extrave(+), Open(-), Self-en(-)\\\cline{2-4}
&13&0&Openness(+), Open(+), Self-en(+)\\\hline


\multirow{3}{*}{Fuel}
&3&1&Agreeab(+), Hedonis(+)\\\cline{2-4}
&4&-1&Agreeab(-), Conscie(+), Self-en(+)\\\cline{2-4}
&8&1&Conscie(+), Extrave(+), Hedonis(-)\\\hline

\multirow{9}{*}{Quality}
&2&0&Neuroti(+), Open(+), Self-en(+), Self-tr(+)\\\cline{2-4}
&4&0&Neuroti(+), Open(-)\\\cline{2-4}
&5&-1&Conscie(+), Neuroti(+)\\\cline{2-4}
&9&0&Agreeab(-), Open(-)\\\cline{2-4}
&10&1&Conscie(+), Extrave(+)\\\cline{2-4}
&12&0&Hedonis(-), Open(-)\\\cline{2-4}
&13&-1&Agreeab(+), Extrave(+), Self-tr(+)\\\cline{2-4}
&14&1&Conscie(+), Openness(+)\\\cline{2-4}
&16&-1&Conserv(-), Hedonis(+), Self-tr(-)\\\hline


\multirow{3}{*}{Style}
&8&-1&Extrave(+), Self-tr(+)\\\cline{2-4}
&13&0&Conscie(+), Self-en(+)\\\cline{2-4}
&15&-1&Openness(+), Conserv(+)\\\hline

Price&1&-1&Neuroti(+), Open(+), Self-en(+)\\\hline


\multirow{6}{*}{Performance}
&1&0&Hedonis(-), Self-tr(-)\\\cline{2-4}
&2&0&Conserv(-), Self-en(-)\\\cline{2-4}
&8&-1&Extrave(+), Conserv(+)\\\cline{2-4}
&10&0&Neuroti(+), Openness(+)\\\cline{2-4}
&12&-1&Extrave(+), Openness(-), Open(-), Self-tr(-)\\\cline{2-4}
&17&-1&Conscie(+), Hedonis(-), Open(-), Self-en(-)\\\hline

\multirow{6}{*}{Durability}
&1&1&Agreeab(-), Conserv(-), Self-en(-)\\\cline{2-4}
&2&0&Conscie(+), Openness(+)\\\cline{2-4}
&7&-1&Extrave(+), Openness(+)\\\cline{2-4}
&10&-1&Neuroti(+), Self-en(+)\\\cline{2-4}
&13&1&Agreeab(+), Neuroti(+)\\\cline{2-4}
&14&0&Agreeab(+), Conscie(+), Open(-), Self-en(-)\\\hline
\end{tabular}
\begin{tablenotes}
\small
\item * label: 1 positive 0 neutral -1 negative
\end{tablenotes}
\end{table*}

==> tbl/tbl_cluster_pattern_2.tex <==
\providecommand{\e}[1]{\ensuremath{\times 8^{#1}}}
\begin{table*}[ht!]
\label{tbl:pattern}
\caption{Patterns in clusters for different features}
\centering
\begin{tabular}{|l|c|l|l|} \hline
Feature & Cluster \#.& Label & Significant traits \\\hline
%Safety
\multirow{7}{*}{Safety} 
&4&pos&Self-en(+), Self-tr(+)\\\cline{2-4}
&6&pos&Agreeab(+)\\\cline{2-4}
&7&neg&Neuroti(+), Open(+), Self-tr(+)\\\cline{2-4}
&9&pos&Open(-)\\\cline{2-4}
&11&neu&Conscie(+), Open(-)\\\cline{2-4}
&12&neu&Extrave(+), Open(-), Self-en(-)\\\cline{2-4}
&13&neu&Openness(+), Open(+), Self-en(+)\\\cline{2-4}
&14&pos&Hedonis(-)\hline


\multirow{3}{*}{Fuel}
&0&neu&Conserv(+)\\\cline{2-4}
&3&pos&Agreeab(+), Hedonis(+)\\\cline{2-4}
&4&neg&Agreeab(-), Conscie(+), Self-en(+)\\\cline{2-4}
&8&pos&Conscie(+), Extrave(+), Hedonis(-)\hline

\multirow{9}{*}{Quality}
&0&pos&Openness(+)\\\cline{2-4}
&1&pos&Self-en(-)\\\cline{2-4}
&2&neu&Neuroti(+), Open(+), Self-en(+), Self-tr(+)\\\cline{2-4}
&4&neu&Neuroti(+), Open(-)\\\cline{2-4}
&5&neg&Conscie(+), Neuroti(+)\\\cline{2-4}
&9&neu&Agreeab(-), Open(-)\\\cline{2-4}
&10&pos&Conscie(+), Extrave(+)\\\cline{2-4}
&11&pos&Openness(+)\\\cline{2-4}
&12&neu&Hedonis(-), Open(-)\\\cline{2-4}
&13&neg&Agreeab(+), Extrave(+), Self-tr(+)\\\cline{2-4}
&14&pos&Conscie(+), Openness(+)\\\cline{2-4}
&15&neg&Neuroti(+)\\\cline{2-4}
&16&neg&Conserv(-), Hedonis(+), Self-tr(-)\hline


\multirow{3}{*}{Style}
&3&neg&Self-en(+)\\\cline{2-4}
&4&neu&Neuroti(+)\\\cline{2-4}
&7&pos&Conscie(+)\\\cline{2-4}
&8&neg&Extrave(+), Self-tr(+)\\\cline{2-4}
&11&neu&Conserv(+)\\\cline{2-4}
&12&neg&Conscie(+)\\\cline{2-4}
&13&neu&Conscie(+), Self-en(+)\\\cline{2-4}
&14&pos&Self-en(-)\\\cline{2-4}
&15&neg&Openness(+), Conserv(+)\\\cline{2-4}
&16&pos&Self-en(+)\hline

Price&1&neg&Neuroti(+), Open(+), Self-en(+)\hline
Luxury&1&neu&Self-en(+)\hline

\multirow{6}{*}{Performance}
&0&neu&Self-tr(+)\\\cline{2-4}
&1&neu&Hedonis(-), Self-tr(-)\\\cline{2-4}
&2&neu&Conserv(-), Self-en(-)\\\cline{2-4}
&4&neg&Conscie(+)\\\cline{2-4}
&5&neg&Conscie(-)\\\cline{2-4}
&8&neg&Extrave(+), Conserv(+)\\\cline{2-4}
&9&neg&Agreeab(-)\\\cline{2-4}
&10&neu&Neuroti(+), Openness(+)\\\cline{2-4}
&11&pos&Hedonis(-)\\\cline{2-4}
&12&neg&Extrave(+), Openness(-), Open(-), Self-tr(-)\\\cline{2-4}
&15&neu&Openness(+)\\\cline{2-4}
&17&neg&Conscie(+), Hedonis(-), Open(-), Self-en(-)\hline

\multirow{6}{*}{Durability}
&0&pos&Openness(+)\\\cline{2-4}
&1&pos&Agreeab(-), Conserv(-), Self-en(-)\\\cline{2-4}
&2&neu&Conscie(+), Openness(+)\\\cline{2-4}
&4&pos&Open(-)\\\cline{2-4}
&6&neg&Openness(+)\\\cline{2-4}
&7&neg&Extrave(+), Openness(+)\\\cline{2-4}
&8&neg&Self-tr(+)\\\cline{2-4}
&9&neu&Self-tr(-)\\\cline{2-4}
&10&neg&Neuroti(+), Self-en(+)\\\cline{2-4}
&11&pos&Neuroti(+)\\\cline{2-4}
&13&pos&Agreeab(+), Neuroti(+)\\\cline{2-4}
&14&neu&Agreeab(+), Conscie(+), Open(-), Self-en(-)\\\cline{2-4}
&15&pos&Hedonis(-)\\\cline{2-4}
&16&neu&Self-en(+)\hline
\end{tabular}
\begin{tablenotes}
\small
\item * label: 1 positive 0 neutral -1 negative
\end{tablenotes}
\end{table*}

==> tbl/tbl_clustering_results.tex <==
\providecommand{\e}[1]{\ensuremath{\times 8^{#1}}}
\begin{table*}[ht!]
\label{tbl:pattern}
\caption{Patterns in clusters for different features}
\centering
\begin{tabular}{|l|c|l|l|} \hline
Feature & Cluster \#.& Label & Significant traits \\\hline
%Safety
\multirow{5}{*}{Safety} 
&4&1&Self-en(+), Self-tr(+)\\\cline{2-4}
&7&-1&Neuroti(+), Open(+), Self-tr(+)\\\cline{2-4}
&11&0&Conscie(+), Open(-)\\\cline{2-4}
&12&0&Extrave(+), Open(-), Self-en(-)\\\cline{2-4}
&13&0&Openness(+), Open(+), Self-en(+)\\\hline


\multirow{3}{*}{Fuel}
&3&1&Agreeab(+), Hedonis(+)\\\cline{2-4}
&4&-1&Agreeab(-), Conscie(+), Self-en(+)\\\cline{2-4}
&8&1&Conscie(+), Extrave(+), Hedonis(-)\\\hline

\multirow{9}{*}{Quality}
&2&0&Neuroti(+), Open(+), Self-en(+), Self-tr(+)\\\cline{2-4}
&4&0&Neuroti(+), Open(-)\\\cline{2-4}
&5&-1&Conscie(+), Neuroti(+)\\\cline{2-4}
&9&0&Agreeab(-), Open(-)\\\cline{2-4}
&10&1&Conscie(+), Extrave(+)\\\cline{2-4}
&12&0&Hedonis(-), Open(-)\\\cline{2-4}
&13&-1&Agreeab(+), Extrave(+), Self-tr(+)\\\cline{2-4}
&14&1&Conscie(+), Openness(+)\\\cline{2-4}
&16&-1&Conserv(-), Hedonis(+), Self-tr(-)\\\hline


\multirow{3}{*}{Style}
&8&-1&Extrave(+), Self-tr(+)\\\cline{2-4}
&13&0&Conscie(+), Self-en(+)\\\cline{2-4}
&15&-1&Openness(+), Conserv(+)\\\hline

Price&1&-1&Neuroti(+), Open(+), Self-en(+)\\\hline


\multirow{6}{*}{Performance}
&1&0&Hedonis(-), Self-tr(-)\\\cline{2-4}
&2&0&Conserv(-), Self-en(-)\\\cline{2-4}
&8&-1&Extrave(+), Conserv(+)\\\cline{2-4}
&10&0&Neuroti(+), Openness(+)\\\cline{2-4}
&12&-1&Extrave(+), Openness(-), Open(-), Self-tr(-)\\\cline{2-4}
&17&-1&Conscie(+), Hedonis(-), Open(-), Self-en(-)\\\hline

\multirow{6}{*}{Durability}
&1&1&Agreeab(-), Conserv(-), Self-en(-)\\\cline{2-4}
&2&0&Conscie(+), Openness(+)\\\cline{2-4}
&7&-1&Extrave(+), Openness(+)\\\cline{2-4}
&10&-1&Neuroti(+), Self-en(+)\\\cline{2-4}
&13&1&Agreeab(+), Neuroti(+)\\\cline{2-4}
&14&0&Agreeab(+), Conscie(+), Open(-), Self-en(-)\\\hline
\end{tabular}
\end{table*}

==> tbl/tbl_constraints_all.tex <==
\begin{table}[h]
\label{tbl:constraint}
\caption{Number of constraints}
\centering
\begin{tabular}{|c|c|c|} \hline
   & MLs & CLs \\ \hline
Safety & 71844 & 39312 \\ \hline
Fuel &62481 & 33660   \\ \hline
Quality & 43002	&36001\\ \hline
Style & 75351	&37224\\ \hline
Price & 89959	&20256 \\ \hline
Luxury & 141477	&11704\\ \hline
Performance & 43621	&29532\\ \hline
Durability & 34902	&34476 \\\hline
\end{tabular}
\end{table}

==> tbl/tbl_constraints_split.tex <==
\begin{table}[h]
\label{tbl:constraint}
\caption{Number of constraints}
\centering
\begin{tabular}{|c|c|c|} \hline
   & MLs & CLs \\ \hline
Safety	&50151	&27664\\ \hline
Fuel	&41796	&23545\\ \hline
Quality	&30123	&25488\\ \hline
Style	&50188	&26840\\ \hline
Price	&61506	&13960\\ \hline
Luxury	&98056	&7974\\ \hline
Performance	&29071	&20384\\ \hline
Durability	&24991	&24464\\ \hline
\end{tabular}
\end{table}

==> tbl/tbl_durability_clustering.tex <==
\begin{table}[h]
\label{tbl:durability_pos}
\caption{Durability(+)}
\centering
\begin{tabular}{|l|c|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.70&	-0.018&	0.24\\ \hline
Consci.	&0.76&	0.001&	0.93\\ \hline
Extro.	&0.54&	-0.004&	0.79\\ \hline
Neuro.	&0.72&	-0.001&	0.97\\ \hline
Openn.	&0.76&	-0.007&	0.52\\ \hline
Conser.	&0.60&	-0.014&	0.34\\ \hline
Hedon.	&0.53&	-0.038&	0.028 *\\ \hline
Open.	&0.59&	-0.024&	0.07\\ \hline
Slf-en.	&0.53&	-0.026&	0.06\\ \hline
Slf-tr.	&0.74&	-0.020&	0.11\\ \hline
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:durability_neg}
\caption{Durability(-)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.72&	0.005&	0.73\\ \hline
Consci.	&0.77&	0.019&	0.09\\ \hline
Extro.	&0.55&	0.009&	0.49\\ \hline
Neuro.	&0.74&	0.014&	0.33\\ \hline
Openn.	&0.77&	0.0001&	0.97\\ \hline
Conser.	&0.62&	0.012&	0.37\\ \hline
Hedon.	&0.58&	0.004&	0.8\\ \hline
Open.	&0.61&	0.001&	0.96\\ \hline
Slf-en.	&0.58&	0.026&	0.04 *\\ \hline
Slf-tr.	&0.76&	-0.003&	0.77\\ \hline
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:durability_neu}
\caption{Durability(neutral)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.72&	0.009&	0.55\\ \hline
Consci.	&0.74&	-0.018&	0.11\\ \hline
Extro.	&0.54&	-0.006&	0.67\\ \hline
Neuro.	&0.71&	-0.013&	0.38\\ \hline
Openn.	&0.78&	0.005&	0.6\\ \hline
Conser.	&0.61&	0.0001&	0.99\\ \hline
Hedon.	&0.60&	0.025&	0.13\\ \hline
Open.	&0.63&	0.018&	0.16\\ \hline
Slf-en.	&0.55&	-0.004&	0.77\\ \hline
Slf-tr.	&0.78&	0.018&	0.09\\ \hline
\end{tabular}
\end{table}


==> tbl/tbl_fuel_clustering.tex <==
\begin{table}[h]
\label{tbl:fuel_pos}
\caption{Fuel(+)}
\centering
\begin{tabular}{|l|c|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.72&-0.004&0.77\\ \hline
Consci.&0.75&0.005&0.637\\ \hline
Extro.&0.54&0.007&0.517\\ \hline
Neuro.&0.72&0.002&0.897\\ \hline
Open.&0.77&-0.003&0.7\\ \hline
Conser.&0.61&0.007&0.55\\ \hline
Hedon.&0.57&0.005&0.71\\ \hline
Open&0.61&-0.001&0.9\\ \hline
Slf-en.&0.54&0.009&0.4	\\ \hline
Slf-tr.&0.77&-0.013&0.19	\\ \hline
\end{tabular}
\end{table}

\begin{table}[h]
\label{tbl:fuel_neg}
\caption{Fuel(-)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.70&-0.01&0.51	\\ \hline
Consci.&0.77&0.01&0.32	\\ \hline
Extro.&0.59&0.05&0.006	*\\ \hline
Neuro.&0.73&0.004&0.83	\\ \hline
Openn.&0.77&0.004&0.74	\\ \hline
Conser.&0.64&0.02&0.12	\\ \hline
Hedon.&0.66&0.09& $< 0.0001$	***\\ \hline
Open.&0.67&0.06& 0.0002	**\\ \hline
Slf-en.&0.63&0.08& $< 0.0001$ ***\\ \hline
Slf-tr.&0.74&-0.02&0.1\\ \hline
\end{tabular}
\end{table}

\begin{table}[h]
\label{tbl:fuel_neu}
\caption{Fuel(neutral)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.72&0.0013	&0.94	\\ \hline
Consci.&0.75&0	&1	\\ \hline
Extro.&0.52&-0.02	&0.15	\\ \hline
Neuro.&0.72	&0.0006	&0.97	\\ \hline
Open.&0.76&	-0.0113	&0.31	\\ \hline
Conser.&0.61&	-0.0047	&0.77	\\ \hline
Hedon.&0.50	&-0.07&	0.0003 **\\ \hline
Open.&0.56&	-0.06	&0.0001	**\\ \hline
Slf-en.&0.50	&-0.05	&0.0006	**\\ \hline
Slf-tr.&0.75	&-0.01	&0.38	\\ \hline
\end{tabular}
\end{table}

==> tbl/tbl_luxury_clustering.tex <==
\begin{table}[h]
\label{tbl:luxury_pos}
\caption{Luxury(+)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.67&	-0.045&	0.32\\ \hline	
Consci.	&0.78&	0.026&	0.35\\ \hline
Extro.	&0.60&	0.057&	0.14\\ \hline
Neuro.	&0.70&	-0.026&	0.5\\ \hline
Openn.	&0.75&	-0.025&	0.27\\ \hline	
Conser.	&0.67&	0.061&	0.17\\ \hline
Hedon.	&0.62&	0.045&	0.36\\ \hline	
Open.	&0.65&	0.040&	0.31\\ \hline	
Slf-en.	&0.68&	0.126&	0.006	*\\ \hline
Slf-tr.	&0.72&	-0.043&	0.3\\ \hline	
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:luxury_neg}
\caption{Luxury(-)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.72&	0.003&	0.80\\ \hline
Consci.&	0.75&	-0.001&	0.87\\ \hline
Extro.	&0.54&	-0.005&	0.64\\ \hline
Neuro.	&0.72&	-0.000&	0.99\\ \hline
Openn.	&0.77&	0.002&	0.81\\ \hline
Conser.	&0.61&	-0.001&	0.88\\ \hline
Hedon.	&0.56&	-0.009&	0.48\\ \hline
Open.&	0.61&	-0.004&	0.7\\ \hline
Slf-en.&	0.54&	-0.013&	0.2\\ \hline
Slf-tr.&	0.76&	0.004&	0.59\\ \hline
\end{tabular}
\end{table}



\begin{table}[h]
\label{tbl:luxury_neu}
\caption{Luxury(neutral)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&	0.70&	-0.012&	0.69\\ \hline
Consci.&	0.76&	0.003&	0.89\\ \hline	
Extro.&	0.57&	0.031&	0.21\\ \hline	
Neuro.	&0.74&	0.014&	0.65	\\ \hline
Openn.	&0.76&	-0.009&	0.64\\ \hline	
Conser.&	0.60&	-0.015&	0.57\\ \hline	
Hedon.	&0.66&	0.09&	0.01	*\\ \hline
Open.&0.64&	0.025&	0.38\\ \hline	
Slf-en.&	0.65&	0.099&	0.0008	*\\ \hline
Slf-tr.&	0.72&	-0.036&	0.1	\\ \hline
\end{tabular}
\end{table}

==> tbl/tbl_performance_clustering.tex <==
\begin{table}[h]
\label{tbl:performance_pos}
\caption{Performance(+)}
\centering
\begin{tabular}{|l|c|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&	0.69&	-0.027&	0.17	\\ \hline
Consci.&	0.78&	0.021&	0.15\\ \hline	
Extro.	&0.56&	0.017	&0.3	\\ \hline
Neuro.&	0.72&	-0.0001	&0.99\\ \hline	
Openn.	&0.77&	-0.002	&0.82	\\ \hline
Conser.	&0.62&	0.009	&0.62\\ \hline	
Hedon.	&0.63&	0.053&	0.01	*\\ \hline
Open.	&0.66&	0.049&	0.004 **\\ \hline
Slf-en.	&0.61&	0.056&	0.003 **\\ \hline
Slf-tr.	&0.75&	-0.012&	0.4532	\\ \hline
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:performance_neg}
\caption{Performance(-)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.72&	0.005&	0.66\\ \hline	
Consci.&	0.75&	-0.004&	0.64\\ \hline	
Extro.&	0.53&	-0.011&	0.33	\\ \hline
Neuro.&	0.72&	-0.004&	0.75\\ \hline	
Openn.&	0.77&	-0.004&	0.62	\\ \hline
Conser.&	0.60&	-0.009&	0.41\\ \hline	
Hedon.&	0.56&	-0.017&	0.23\\ \hline	
Open.&	0.59&	-0.022&	0.0513	\\ \hline
Slf-en.&	0.53&	-0.022&	0.0540\\ \hline	
Slf-tr.&	0.75&	-0.005&	0.5818\\ \hline	
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:performance_neu1}
\caption{Performance(neutral)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.58&	-0.13&	$<0.0001$ ***\\ \hline
Consci.	&0.69&	-0.067&	$<0.0001$ ***\\ \hline
Extro.	&0.48&	-0.063&	0.0005	**\\ \hline
Neuro.	&0.63&	-0.093&	$<0.0001$ ***\\ \hline
Openn.	&0.73&	-0.045&	0.0002	**\\ \hline
Conser.	&0.57&	-0.044&	0.008	*\\ \hline
Hedon.	&0.50&	-0.075&	0.0002	**\\ \hline
Open.	&0.54&	-0.076&	$<0.0001$ ***\\ \hline
Slf-en.	&0.51&	-0.043&	0.0059	*\\ \hline
Slf-tr.	&0.66&	-0.098&	$<0.0001$ ***\\ \hline
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:performance_neu2}
\caption{Performance(neutral)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.83&	0.11&		$<0.0001$ ***\\ \hline
Consci.	&0.80&	0.042&		0.002	**\\ \hline
Extro.	&0.60&	0.058&		0.0009	**\\ \hline
Neuro.	&0.80&	0.08&		$<0.0001$ ***\\ \hline
Openn.	&0.82&	0.047&		$<0.0001$ ***\\ \hline
Conser.	&0.66&	0.046&		0.005	*\\ \hline
Hedon.	&0.62&	0.05&		0.02	*\\ \hline
Open.	&0.68&	0.065&		$<0.0001$ ***\\ \hline
Slf-en.	&0.59&	0.035&		0.053	\\ \hline
Slf-tr.	&0.86&	0.097&		$<0.0001$ ***\\ \hline
\end{tabular}
\end{table}

==> tbl/tbl_price_clustering.tex <==
\begin{table}[h]
\label{tbl:price_pos}
\caption{Price(+)}
\centering
\begin{tabular}{|l|c|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.71&-0.002&0.88\\ \hline	
Consci.&0.75&-0.006&0.48\\ \hline	
Extro.&0.53&-0.008&0.46	\\ \hline
Neuro.&0.72&-0.005&0.7\\ \hline	
Openn.&0.77&-0.0001&0.96	\\ \hline
Conser.&0.60&-0.012&0.23	\\ \hline
Hedon.&0.57&-0.006&0.63	\\ \hline
Open.&0.61&-0.009&0.38\\ \hline	
Slf-en.&0.54&-0.008&0.43	\\ \hline
Slf-tr.&0.75&-0.007&0.46\\ \hline	
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:price_neg}
\caption{Price(-)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.72&	0.001&	0.95\\ \hline	
Consci.	&0.80&	0.048&	0.03 *\\ \hline
Extro.	&0.60&	0.054&	0.03 *\\ \hline
Neuro.	&0.76&	0.043&	0.13\\ \hline	
Openn.	&0.78&	0.007&	0.64\\ \hline	
Conser.	&0.69&	0.074&	0.005 *\\ \hline
Hedon.	&0.64	&0.068&	0.04 *\\ \hline
Open.	&0.69&	0.076&	0.004 **\\ \hline
Slf-en	&0.63&	0.079&	0.01 *\\ \hline
Slf-tr	&0.81&	0.048&	0.02 *\\ \hline
\end{tabular}
\end{table}

\begin{table}[h]
\label{tbl:price_neu}
\caption{Price(neutral)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.72&	0.005&	0.78\\ \hline
Consci.	&0.76&	0.002&	0.87\\ \hline
Extro.	&0.55&	0.006&	0.7\\ \hline
Neuro.	&0.72&	-0.002&	0.92\\ \hline
Openn.	&0.77&	-0.002&	0.87\\ \hline
Conser.	&0.62&	0.012&	0.49\\ \hline
Hedon.	&0.57	&-0.005&	0.79\\ \hline
Open.	&0.61&	-0.001&	0.97\\ \hline
Slf-en.	&0.55&	-0.003&	0.85\\ \hline
Slf-tr.	&0.76&	0.003&	0.82\\ \hline

\end{tabular}
\end{table}



==> tbl/tbl_quality_clustering.tex <==
\begin{table}[h]
\label{tbl:quality_pos}
\caption{Quality(+)}
\centering
\begin{tabular}{|l|c|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.71	&0.003&	0.8	\\ \hline
Consci.&0.75&	0.005&	0.61\\ \hline	
Extro.&0.55&	0.01&	0.4	\\ \hline
Neuro.&0.71&	-0.003&	0.8\\ \hline	
Openn.&0.77&	0.003&	0.66\\ \hline
Conser.&0.61&	0.003&	0.74\\ \hline	
Hedon.&0.59&	0.01&	0.24	\\ \hline
Open.&0.62&0.01&	0.22\\ \hline	
Slf-en&0.56&	0.01&	0.2\\ \hline	
Slf-tr&0.76&0.006&	0.5\\ \hline	
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:quality_neg}
\caption{Quality(-)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.71&-0.005&0.82\\ \hline
Consci.&0.74&-0.012&0.61\\ \hline
Extro.&0.55&0.002&0.40\\ \hline
Neuro.&0.72&0.003&0.80\\ \hline
Openn.&0.77&-0.008&0.66\\ \hline
Conser.&0.62&0.016&0.75\\ \hline
Hedon.&0.59&0.013&0.24\\ \hline
Open.&0.63&0.002&0.22\\ \hline
Slf-en.&0.55&-0.0008&0.2\\ \hline
Slf-tr.&0.75&-0.008&0.51\\ \hline
\end{tabular}
\end{table}

\begin{table}[h]
\label{tbl:quality_neu}
\caption{Quality(neutral)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.71&-0.0004&0.97\\ \hline	
Consci.&0.76&0.002&0.88\\ \hline	
Extro.&0.53&-0.015&0.27\\ \hline	
Neuro.&0.72&0.002&0.88\\ \hline	
Openn.&0.77&0.001&0.9\\ \hline	
Conser.&0.60&-0.017&0.22\\ \hline	
Hedon.&0.54&-0.033&0.04	*\\ \hline
Open.&0.59&-0.021&0.11\\ \hline	
Slf-en.&0.53&-0.02&0.15\\ \hline
Slf-tr&0.76&-0.003&0.79\\ \hline	
\end{tabular}
\end{table}

==> tbl/tbl_readerdist.tex <==
\begin{table}[h]
\label{tbl:readerdist}
\centering
\begin{tabular}{|c|c|c|} \hline
Traits &Polarity& Number\\ \hline
\multirow{2}{*}{Agreeableness} & + & 114\\ \cline{2-3}
 & - & 121 \\ \hline
 \multirow{2}{*}{Conscientiousness} & + & 158\\ \cline{2-3}
 & - & 100 \\ \hline
 \multirow{2}{*}{Extroversion} & + & 83\\ \cline{2-3}
 & - & 132 \\ \hline
 \multirow{2}{*}{Neutoticism} & + & 186\\ \cline{2-3}
 & - & 93 \\ \hline
 \multirow{2}{*}{Openness} & + & 99\\ \cline{2-3}
 & - & 117 \\ \hline
\multirow{2}{*}{Conservation} & + & 131\\ \cline{2-3}
 & - & 77 \\ \hline
 \multirow{2}{*}{Hedonism} & + & 120\\ \cline{2-3}
 & - & 83 \\ \hline
 \multirow{2}{*}{Openness to change} & + & 113\\ \cline{2-3}
 & - & 117 \\ \hline
 \multirow{2}{*}{Self enhancement} & + & 122\\ \cline{2-3}
 & - & 105 \\ \hline
 \multirow{2}{*}{Self transcendence} & + & 104\\ \cline{2-3}
 & - & 120 \\ \hline
\end{tabular}
\caption{The distribution of Reader based on different traits}
\end{table}


==> tbl/tbl_regression_evaluation.tex <==
\begin{table}[h]
\label{tbl:fuel_pos}
\caption{Fuel(+)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
	&SST	&SSE	&R^2 \\ \hline
Safety	&435.79	&425.25	&0.02\\ \hline
Fuel	&296.51	&302.18	&-0.02\\ \hline
Quality	&342.76	&340.47	&0.01\\ \hline
Style	&276.51	&300.32	&-0.09\\ \hline
Quality	&342.76	&340.47	&0.01\\ \hline
Price	&333.31	&335.38	&-0.01\\ \hline
Luxury	&186.75	&178.18	&0.05\\ \hline
Performance	&289.76	&342.77	&-0.18\\ \hline
Durability	&306.99	&311.41	&-0.01\\ \hline
\end{tabular}
\end{table}


==> tbl/tbl_regression_train.tex <==
\providecommand{\e}[1]{\ensuremath{\times 10^{#1}}}
\small
\begin{table*}[ht!]
\label{tbl:regression}
\caption{Results of the Regression Analysis}
\centering
\begin{tabular}{|c|l|l|l|l|l|l|l|l|} \hline
 &Safety& Fuel & Quality & Style & Price &Luxury & Perf & Durab\\\hline
Agreeableness		&0.32	&-0.78	&-0.51	&0.70	&0.84	&0.01	&-0.46	&-0.11\\\hline
Conscientiousness	&-1.16	&0.02	&0.67	&0.28	&-0.74	&0.27	&0.86	&-0.19\\\hline
Extraversion		&1.21	&-0.42	&0.28	&-0.37	&-0.58	&0.50	&-0.27	&-0.35\\\hline
Neuroticism			&0.97	&-0.09	&-0.59	&-0.25	&-0.23	&-0.19	&0.44	&-0.04\\\hline
Openness			&2.02*	&0.33	&-0.15	&-1.16	&0.34	&-0.75	&-0.61	&-0.02\\\hline
Conservation		&2.10*	&-0.98	&-0.11	&1.04	&-1.50*	&0.18	&-0.37	&-0.37\\\hline
Hedonism			&1.27	&0.10	&-0.44	&0.25	&0.30*	&0.02	&-0.91	&-0.60\\\hline
Openness to change	&-1.83	&-0.18	&0.66	&0.57	&-2.20	&-0.44	&2.28*	&1.15\\\hline
Self-enhancement	&-1.70	&-1.63*	&0.02	&0.23	&-0.03	&2.46***	&1.79*	&-1.15\\\hline
Self-transcendence	&1.34	&2.51*	&1.25	&-2.86**	&-0.67	&-1.13	&-0.15	&-0.28\\\hline
\end{tabular}
\begin{tablenotes}
\small
\item * $p < 0.05$, ** $p < 0.005$, *** $p < 0.0001$
\end{tablenotes}

\end{table*}

==> tbl/tbl_safety_clustering.tex <==
\begin{table}[h]
\label{tbl:safety_pos}
\caption{Safety(+)}
\centering
\begin{tabular}{|l|c|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.\footnotemark &0.747&0.033&0.005 *\\ \hline
Consci.\footnotemark &0.763&0.009&0.31 \\ \hline
Extro.\footnotemark &0.551&0.008&0.46\\ \hline
Neuro.\footnotemark &0.741&0.019&	0.11\\ \hline
Openn.\footnotemark &0.777&0.006&0.44\\ \hline
Conser.\footnotemark &0.631&0.019&0.06\\ \hline
Hedon.\footnotemark&0.558&-0.015&0.27\\ \hline
Open.\footnotemark &0.605&-0.009&0.38\\ \hline
Slf-en.\footnotemark &0.540&-0.011&0.34\\ \hline
Self-tr.\footnotemark &0.783&0.024&0.008*\\ \hline
\end{tabular}
\end{table}
\addtocounter{footnote}{-9}
\footnotetext{Agreeableness}
\addtocounter{footnote}{1}
\footnotetext{Conscientiousness}
\addtocounter{footnote}{1}
\footnotetext{Extroversion}
\addtocounter{footnote}{1}
\footnotetext{Neurotisim}
\addtocounter{footnote}{1}
\footnotetext{Openness}
\addtocounter{footnote}{1}
\footnotetext{Conservation} 
\addtocounter{footnote}{1}
\footnotetext{Hedonism}
\addtocounter{footnote}{1}
\footnotetext{Openness to change}
\addtocounter{footnote}{1}
\footnotetext{Self-enhancement}
\addtocounter{footnote}{1}
\footnotetext{Self-transcendence}

\begin{table}[h]
\label{tbl:safety_neg}
\caption{Safety(-)}
\centering
\begin{tabular}{|l|c|c|c|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&0.654&-0.061&0.0001 **\\ \hline
Consci.&0.737&-0.017&0.12\\ \hline
Extro.&0.528&-0.015&0.27\\ \hline
Neuro.	&0.686&-0.035&0.02*\\ \hline
Openn.&0.760&-0.011&0.26\\ \hline
Conser.&0.576&-0.036&0.008 *\\ \hline
Hedon.&0.601&0.028&0.07\\ \hline
Open.&0.632&0.017&0.13\\ \hline
Slf-en.&0.571&0.020&0.12\\ \hline
Slf-tr.&0.716&-0.044&0.0002 **\\ \hline
\end{tabular}
\end{table}

==> tbl/tbl_style_clustering.tex <==
\begin{table}[h]
\label{tbl:style_pos}
\caption{Style(+)}
\centering
\begin{tabular}{|l|c|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.&	0.67&	-0.04&	0.07	\\ \hline
Consci.&	0.73&	-0.02&	0.2	\\ \hline
Extro.&	0.53&	-0.01&	0.57	\\ \hline
Neuro.&	0.70&	-0.016&	0.4	\\ \hline
Open.&	0.74&	-0.025&	0.04 *\\ \hline
Conser.&	0.62&	0.008&	0.61	\\ \hline
Hedon.&	0.61&	0.034&	0.15553	\\ \hline
Open.&	0.62&	0.002&	0.9	\\ \hline
Slf-en.&	0.57&	0.021&	0.27\\ \hline	
Slf-tr.&	0.72&	-0.043&	0.007 *\\ \hline
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:style_neg}
\caption{Style(-)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.72&	0.0066&	0.70	\\ \hline
Consci.&	0.75&	-0.005&	0.57\\ \hline	
Extro.	&0.54&	-0.003&	0.74\\ \hline	
Neuro.	&0.72&	-0.00002&	0.99\\ \hline	
Open.	&0.77&	0.003&	0.64\\ \hline
Conser.	&0.60&	-0.008	&0.4\\ \hline	
Hedon.	&0.56	&-0.016&	0.22	\\ \hline
Open.	&0.61&	-0.008&	0.39\\ \hline	
Slf-en.	&0.54&	-0.0143&	0.19\\ \hline	
Slf-tr.	&0.77&	0.01&	0.26\\ \hline	
\end{tabular}
\end{table}

\begin{table}[h]
\label{tbl:style_neu1}
\caption{Style(neutral 1)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.82	&0.11&	$<0.0001$	***\\ \hline	
Consci.	&0.85	&0.097&	$<0.0001$	***\\ \hline	
Extro.	&0.65	&0.111&	$<0.0001$	***\\ \hline	
Neuro.	&0.85	&0.123&	$<0.0001$	***\\ \hline	
Openn.	&0.82	&0.045&	0.0001	**\\ \hline	
Conser.	&0.70&	0.085&	0.001	**\\ \hline	
Hedon.	&0.64	&0.06&	0.013	*\\ \hline	
Open.	&0.69&	0.071&	0.001	**\\ \hline	
Slf-en.	&0.62&	0.065&	0.006	*\\ \hline	
Slf-tr.	&0.84&	0.078&	$<0.0001$	***\\ \hline	
\end{tabular}
\end{table}


\begin{table}[h]
\label{tbl:style_neu2}
\caption{Style(neutral 2)}
\centering
\begin{tabular}{|l|c|c|l|} \hline
Traits & $Mean_{c}$ & $Diff$ & $p$ \\ \hline
Agree.	&0.65&	-0.065&	0.003	**\\ \hline
Consci.&	0.73&	-0.026&	0.08	\\ \hline
Extro.	&0.48&	-0.064&	0.001	**\\ \hline
Neuro.	&0.63&	-0.086&	0.0001	**\\ \hline
Openn.	&0.75&	-0.022&	0.12	\\ \hline
Conser.	&0.57&	-0.038&	0.05\\ \hline	
Hedon.	&0.56	&-0.014&	0.53	\\ \hline
Open.&	0.6	&-0.015&	0.41\\ \hline	
Slf-en.	&0.54&	-0.006&	0.72\\ \hline	
Slf-tr.	&0.7&	-0.064&	0.0008	**\\ \hline
\end{tabular}
\end{table}

==> tbl/tbl_svm_majority.tex <==
\begin{table}[h]
\label{tbl:constraint}
\caption{Number of constraints}
\centering
\begin{tabular}{|c|c|c|c|} \hline
&	Majority&	SVM&	p \\\hline
Safety&	61&	61&	0.53\\\hline
Fuel&	57&	58&	0.45\\\hline
Quality&	44&	47&	0.31\\\hline
Style&	63&	63&	0.53\\\hline
Price&	71&	71&	0.53\\\hline
Luxury&	90&	91&	0.41\\\hline
Performance&	46&	50&	0.24\\\hline
Durability&	37&	42&	0.18\\\hline
\end{tabular}
\end{table}

==> tbl/tbl_trait.tex <==
\providecommand{\e}[1]{\ensuremath{\times 8^{#1}}}
\begin{table}
\label{tbl:traits}
\caption{Description of Two Trait Models}
\scriptsize
\centering
\begin{tabular}{| p{1cm} | p{2cm} | p{4cm}|} \hline
Model & Feature & Description\\\hline
 & Openness to experience &  The degree of intellectual curiosity, creativity and a preference for novelty and variety a person has. \\\cline{2-3}
\multirow{5}{1cm}{Big5 Personality Model}& Conscientious &  A tendency to be organized and dependable, show self-discipline, act dutifully, aim for achievement, and prefer planned rather than spontaneous behavior. \\\cline{2-3}
& Extraversion &   Energy, positive emotions, surgency, assertiveness, sociability and the tendency to seek stimulation in the company of others, and talkativeness. \\\cline{2-3}
& Agreeableness &  A tendency to be compassionate and cooperative rather than suspicious and antagonistic towards others. \\\cline{2-3}
& Neuroticism &  The tendency to experience unpleasant emotions easily, such as anger, anxiety, depression, and vulnerability. \\\hline
& Openness to Change &  The desire for independence and new, novel, exciting and challenging experiences. \\\cline{2-3}
 \multirow{5}{1cm}{Schwartz's human basic values}& Self-Enhancement &  The pursuit of self-interests including social status, prestige, resources and personal success through demonstrating competence. \\\cline{2-3}
& Conservation &  Self-restriction and conform to tradition, social expectations and norms;  Pursue safety, harmony and stability; resist to change \\\cline{2-3}
& Hedonism &  Pursuit of pleasure and sensuous gratification for oneself. \\\cline{2-3}
& Self-transcendence &  Concern and pursue the enhancement and protection of the welfare and interests of others as well as the protection for nature. \\\hline
\end{tabular}
\end{table}
